Overwatch: Learning Patterns in Code Edit Sequences

Integrated Development Environments (IDEs) provide tool support to automate many source code editing tasks. Traditionally, IDEs use only the spatial context, i.e., the location where the developer is editing, to generate candidate edit recommendations. However, spatial context alone is often not sufficient to confidently predict the developer's next edit, and thus IDEs generate many suggestions at a location. Therefore, IDEs generally do not actively offer suggestions and instead, the developer is usually required to click on a specific icon or menu and then select from a large list of potential suggestions. As a consequence, developers often miss the opportunity to use the tool support because they are not aware it exists or forget to use it. To better understand common patterns in developer behavior and produce better edit recommendations, we can additionally use the temporal context, i.e., the edits that a developer was recently performing. To enable edit recommendations based on temporal context, we present Overwatch, a novel technique for learning edit sequence patterns from traces of developers' edits performed in an IDE. Our experiments show that Overwatch has 78% precision and that Overwatch not only completed edits when developers missed the opportunity to use the IDE tool support but also predicted new edits that have no tool support in the IDE.

==> acknowledgement.tex <==
\section{ACKNOWLEDGEMENT}



==> algorithms/anti_unification.tex <==
% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\algorithmicdefault{\textbf{default}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algdef{SE}[DEFAULT]{Default}{EndDefault}[0]{\algorithmicdefault}{\algorithmicend\ \algorithmicdefault}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%
\algtext*{EndDefault}%

\begin{algorithm}
  \small
  \begin{algorithmic}[1]
    \Require Two edit sequence patterns $\langle \tpltseq_1=\etplt_1^1\ldots,\etplt_n^1, \tmprel_1 \rangle, \langle \tpltseq_2=\etplt_1^2\ldots,\etplt_n^2, \tmprel_2 \rangle$
    \Ensure A new edit sequence pattern $\langle \tpltseq, \tmprel \rangle$ merged from two given patterns, the cost $C$.
    %
    \Function{AntiUnify}{$
        \langle \tpltseq_1=\etplt_1^1\ldots,\etplt_n^1, \tmprel_1 \rangle,
        \langle \tpltseq_2=\etplt_1^2\ldots,\etplt_n^2, \tmprel_2 \rangle
    $}
      \State $\tmprel,\substitution_1,\substitution_2,\mathsf{CurEqRel}
        \gets \emptyset, \emptyset, \emptyset, \emptyset$
      %
      \For{$i \in \{ 1, \ldots, n\}$}
        \State $\substitution_1', \substitution_2', C', \tplt_{i,\pre} \gets $ \Call{AntiUnifyTemplate}{$\tplt_{i,\pre}^1$, $\tplt_{i,\pre}^2$, $\mathsf{CurEqRel}$}
        \State $
            C, \substitution_1, \substitution_2, \mathsf{CurEqRel} \gets
            C + C',
            \substitution_1 \cup \substitution_1',
            \substitution_2 \cup \substitution_2',
            \mathsf{CurEqRel} \cup \{(\substitution_1(\hole), \substitution_2(\hole))
            \mid \hole \in \tplt_{i,\pre}\}$
        
         \State $\substitution_1', \substitution_2', C', \tplt_{i,\post} \gets $ \Call{AntiUnifyTemplate}{$\tplt_{i,\post}^1$, $\tplt_{i,\post}^2$, $\mathsf{CurEqRel}$}
        \State $C \gets C + C', \substitution_1 \gets \substitution_1 \cup \substitution_1', \substitution_2 \gets \substitution_2 \cup \substitution_2', \mathsf{CurEqRel} \gets \mathsf{CurEqRel} \cup \{(\substitution_1(\hole), \substitution_2(\hole))|\hole \in \tplt_{i,\post}\}$
        \State Add $\tplt_{i,\pre} \to \tplt_{i,\post}$ to $\tpltseq$
      \EndFor
      \State Add relations to $\tmprel$ based on $\substitution_1, \substitution_2, \tmprel_1, \tmprel_2$
      \State $C \gets \frac{C}{|\tpltseq_1| + |\tpltseq_2|}$
      \State \Return $\langle \tpltseq, \tmprel \rangle, C$
      \EndFunction
    \Function{AntiUnifyChildren}{$c_1^1,\dots,c_p^1$, $c_1^2,\dots,c_q^2$, $\mathsf{CurEqRel}$} 
    % \Comment{Find a template  and $\substitution_1, \substitution_2$ such that 1) $\substitution_1(c_1,\dots,c_r) = c_1^1,\dots,c_p^1, \substitution_2(c_1,\dots,c_r) = c_1^2,\dots,c_q^2$, and 2) the cost $C'=\sum_{\hole \in \tplt \wedge (\substitution_1(H), \substitution_2(H)\notin \mathsf{CurEqRel}} \cost(\hole)$ is minimized.}
        \For{$1 \le i \le p$, $1 \le j \le q$} \Comment{Dynamic programming}
            \If{$c_i^1$ is already a hole}
                \State $C_1 \gets f_{i-1,j}+0.5$ if $(c_i^1, \epsilon) \not \in \mathsf{CurEqRel}$, otherwise, $C_1 \gets 0$
            \Else
                 \State $C_1 \gets f_{i-1,j}+|c_i^1|+0.5$ if $(c_i^1, \epsilon) \not \in \mathsf{CurEqRel}$, otherwise, $C_1 \gets 0$
            \EndIf
            \If{$c_j^2$ is already a hole}
                \State $C_2 \gets f_{i,j-1}+0.5$ if $(\epsilon, c_j^2) \not \in \mathsf{CurEqRel}$, otherwise, $C_2 \gets 0$
            \Else
                \State $C_2 \gets f_{i,j-1}+|c_j^2|+0.5$ if $(\epsilon, c_j^2) \not \in \mathsf{CurEqRel}$, otherwise, $C_2 \gets 0$
            \EndIf
            \State $C_3 \gets f_{i-1,j-1}+$\Call{AntiUnifyTemplate}{$c_i^1$, $c_j^2$, $\mathsf{CurEqRel}$}\code{.cost}$)$
            \Switch{$C_1, C_2, C_3$}
                \Case{$C_1 \le C_2 \wedge C_1 \le C_3$}
                    \State $f_{i,j} \gets C_1$ \Comment{Create a hole $\hole$ such that $\substitution_1(\hole)=c_i^1, \substitution_2(\hole)=\epsilon$}
                \EndCase
                \Case{$C_2 \le C_1 \wedge C_2 \le C_3$}
                    \State $f_{i,j} \gets C_2$ \Comment{Create a hole $\hole$ such that $\substitution_1(\hole)=\epsilon, \substitution_2(\hole)=c_j^2$}
                \EndCase
                \Default 
                    \State $f_{i,j} \gets C_3$ \Comment{Get template $\tplt'$ from AntiUnifyTemplate such that $\substitution_1(\tplt')=c_i^1, \substitution_2(\tplt')=c_j^2$}
                \EndDefault
            \EndSwitch
        \EndFor
        \State $C' \gets f_{p,q}$
        \State Get $\tplt, \substitution_1, \substitution_2$ from the optimal trace of dynamic programming.
        \State \Return $\substitution_1, \substitution_2, C', \tplt$
    \EndFunction
    
    \Function{AntiUnifyTemplate}{$T_1$, $T_2$, $\mathsf{CurEqRel}$} \Comment{Returns two substitutions, the cost, and the anti-unified edit template.}
        \Switch{$T_1, T_2$}
            \Case{At least one of $T_1, T_2$ is a hole or \code{$T_1$.root $\neq$ $T_2$.root}}
                \State $\substitution_1 \gets \{\hole \mapsto T_1\}, \substitution_2 \gets \{\hole \mapsto T_2\}$
                \State $C' \gets \cost(\hole, \substitution_1, \substitution_2)$ if $(T_1, T_2) \notin \mathsf{CurEqRel}$, otherwise, $C' \gets 0$ 
                \State \Return $\substitution_1, \substitution_2, C', \hole$ 
            \EndCase
            \Case{$T_1 = T_2$}
                \State \Return $\varnothing, \varnothing, 0, T_1$
            \EndCase
            \Default \Comment{\code{$T_1$.root = $T_2$.root}}
                \State \Return \Call{AntiUnifyChildren}{$T_1$\code{.children}, $T_2$\code{.children}, $\mathsf{CurEqRel}$} 
            \EndDefault
        \EndSwitch
    \EndFunction
  \end{algorithmic}
  \caption{The procedure of anti-unification and cost computation}
  \label{algo:anti-unification}
\end{algorithm}

==> extra_stuff.tex <==

\begin{figure*}[t]
  \small
%   \includegraphics{figures/overview_draft.png}
%   \tikzset{
%     artifact/.style = {draw, rectangle, minimum width=1.5cm, minimum height=0.75cm},
%     process/.style = {draw=none}
%   }
%   \begin{tikzpicture}
%     \node[artifact, double, xshift=-3cm] (sessions) {\tabular{c}Development\\Sessions\endtabular};
%     \node[artifact] (data) {\tabular{c}Edits\endtabular};
%     \node[process, xshift=0cm, yshift=-1.2cm] (expand) {Extract};
%     \node[artifact, xshift=4.5cm, yshift=-1.2cm] (edit graph) {\tabular{c}Edit\\Graph\endtabular};
%     \node[process, xshift=2cm] (clustering) {\tabular{c}Hierarchical\\Clustering\endtabular};
%     \node[artifact, xshift=4.5cm] (clusters) {Edit Patterns};
%     \node[process, xshift=7cm] (summarization) {Summarize};
%     \node[artifact, xshift=9.25cm] (summary) {\tabular{c}Temporal Edit\\ Summary\endtabular};
%     \node[process, xshift=12cm] (querying) {\tabular{c}Semi-automated\\Pattern Mining\endtabular};
%     \node[artifact, double, xshift=12cm, yshift=-1.2cm] (esp) {\tabular{c}Temporal Edit\\Patterns\endtabular};

%     \node[xshift=-1.2cm, yshift=0.8cm] (top left) {};
%     \node[xshift=10.5cm, yshift=0.8cm] (top mid left) {};
%     \node[xshift=11cm, yshift=0.8cm] (top mid right) {};
%     \node[xshift=16.5cm, yshift=0.8cm] (top right) {};

%     % \draw[-,thick,dashed] (top left) edge node[above] {Pre-compute once} (top mid left);
%     % \draw[-,thick,dashed] (top mid right) edge node[above] {Query many times} (top right);
%     \draw[->] (sessions) -- (data);
%     \draw[->] (data) -- (expand);
%     \draw[->] (expand) -- (edit graph);
%     \draw[->] (data) -- (clustering);
%     \draw[->] (clustering) -- (clusters);
%     \draw[->] (edit graph) -| (summarization);
%     \draw[->] (clusters) -- (summarization);
%     \draw[->] (summarization) -- (summary);
%     \draw[->] (summary) -- (querying);
%     \draw[->] (querying) -- (esp);
%   \end{tikzpicture}
%  \vspace{-4ex}
  % \arsays{TODO: Incorporate Ameya's pictures in nodes}
\end{figure*}

\ignore{
\Cref{fig:techniqueOverview} shows the high-level overview of \technique.
%
The \technique is composed of two distinct phases: the \emph{pre-computation
phase} and the \emph{guided exploration phase}.
%
The pre-computation phase is completely automated, while the guided querying
phase includes both automated and user-guided components.
%
% The user input is used, not only to provide the query, but also to guide the
% query answering mechanism.
%
In the pre-computation phase, the procedure takes as input a set of
\emph{development sessions}---each development session is the collection of
all syntactically correct versions of a source code file produced as a
developer is editing code.
%
From the sessions, the pre-computation phase extracts and condense the
temporal information of the developers' edit actions into a summary.
%
% information about common editing patterns into an artifact called \emph{edit
% sequence summary}.

\gustavo{I like these examples of guided-search but I think it may lead to some disappointment later on in the studies.}
With the summary, the guided exploration can be used to answer
questions about temporal editing patterns.
% user queries to produce edit sequence patterns.
%
A user may investigate questions like
%
``how often do developers modify a function's return type and what are the
actions that precede it?''
%
or
``do developers perform the extract constant refactoring manually, and if so,
in what different ways?''
%
Together, \technique and the user will be able to succinctly capture this
behavior into a \emph{temporal edit pattern}.
% \technique would respond to such queries by producing a set of edit sequence
% patterns which succinctly capture this behavior, along with their frequencies.
% 
Using this guided exploration mechanism a toolsmith\gustavo{Let's make this uniform across the paper... right now we have tool builders, and IDE designers, Ameya, what is the common name in the community?} can obtain
information that might be valuable for planning or prioritizing new features.
}

% In Section~\ref{sec:prelims}, we start with some preliminaries and
% definitions about edit patterns and temporal edit patterns.
%
% In Sections~\ref{sec:precompute}, we describe \technique's mining approach.

% We start by describing the inputs and outputs to our technique.
%

\ignore{
\noindent\textbf{Edit Patterns and Edit Sequence Patterns.}
We represent similar edits using \emph{edit patterns}.
%
An edit pattern uses an edit template $\etplt = \tplt^{\mathsf{pre}} \to
\tplt^{\mathsf{post}}$ to represent version $\vpre$ and $\vpost$. 
%
The edit template $\etplt$ contains two templates $\tplt^{\mathsf{pre}}$ and
$\tplt^{\mathsf{post}}$, which are two ASTs with holes.

An \emph{edit sequence pattern} is a union-free regular expression of edit patterns, i.e., a sequence of concatenation of edit patterns, some of which contain a Kleene star. 
We represent each edit sequence pattern by a sequence of edit templates representing edit patterns, and a \emph{temporal information}, which is the equality relation over every pair of holes among all edit templates. 
Formally, an edit sequence pattern contains two components, a edit template sequence $\tpltseq$ and a temporal information $\tmprel$:
\begin{itemize}
    \item We define an edit template sequence as $\tpltseq = \etplt_1^{[*]} \ldots \etplt_n^{[*]}$, where $[*]$ denotes a optional Kleene star. Each template $\etplt_i = \tplt_i^{\mathsf{pre}} \to \tplt_i^{\mathsf{post}}$ describes an edit pattern.
    \item We define a temporal information is as $\tmprel: 2^{\holespace \times \holespace}$, where $\holespace$ is the space of holes. 
    $\tmprel$ can be seen as the equivalence relation over pairs of holes in the template sequence $\tpltseq$.
\end{itemize}

\begin{example}
\label{exp:def_tts}
Suppose we mine a edit sequence $\edit_1, \edit_2$, where $\edit_1 = \version_0 \to \version3, \edit_2 = \version_3 \to \version_4$ shown in Figure~\ref{fig:dev-session} and we learn an edit sequence pattern containing an edit template sequence $\tpltseq= \etplt_1\etplt_2$ and $\tmprel$, where  
\begin{align*}
\etplt_1 &= \hole_{1}\ \hole_{2}\ \to\ \hole_{3}\textit{ public }\hole_{4}\ \hole_{5}\ \hole_{6}\ \hole_{7}\\
\etplt_2 &= \hole_{8}\ \to\ \hole_{9},\ \hole_{10}\ \hole_{11}\\
\tmprel &= \{(\hole_{1}, \hole_{3}), (\hole_{2}, \hole_{7}), (\hole_{4}, \hole_{10}), (\hole_{8}, \hole_{9}), \ldots\},
\end{align*}
where we omit reflexive and symmetric relations in $\tmprel$ for simplicity.
Notice that from $\tmprel$, we know that the property type $\hole_{4}$ should be equal to the argument type $\hole_{10}$.
\end{example}


\noindent\textbf{Match between Edits and Edit Templates}
We say a version $\version$ matches a template $\tplt$ if we can find a \textit{unique} substitution $\delta$, which is a map from holes to a sequence of concrete ASTs, such that substituting every hole by $\delta$ in $\tplt$ gives us $\version$, formally, $\delta(\tplt) = \version$.
Furthermore, we denote the match between an edit $\edit = \vpre \to \vpost$ and an edit template $\etplt = \tplt^{\mathsf{pre}} \to \tplt^{\mathsf{post}}$ as $\delta(\etplt) = \edit$, if we can find a \textit{unique} substitution $\delta$, such that $\delta(\tplt^{\mathsf{pre}}) = \vpre \wedge \delta(\tplt^{\mathsf{post}}) = \vpost$.
% We use a search algorithm to enumerate all possible substitutions.
\begin{example}
Considering $\etplt_1$ of the edit sequence pattern in Example~\ref{exp:def_tts}, we can find a unique substitution $\delta_1$,
\begin{align*}
    \delta_1 = \{&\hole_{1} \mapsto \textit{class Node \{}, \hole_{2} \mapsto \textit{Node () \{\} \}}, \hole_{3} \mapsto \textit{class Node \{}\\
    &\hole_4 \mapsto \textit{str}, \hole_5 \mapsto \textit{Id}, \hole_6 \mapsto \textit{\{get; set;\}}, \hole_{7} \mapsto \textit{Node () \{\} \}}\},
\end{align*}
such that $\delta_1(\etplt_1) = \edit_1$.
\end{example}

\noindent\textbf{Usage of Edit Sequence Patterns}\todo{reflect the general function relation}
\todo{reflect the Kleene star}
We can use an edit sequence pattern to predict the post version of the $(i+1)$th edit $\edit_{i+1} = \version_{i} \to ?$, if we can find a \textit{unique} substitution $\delta_{\text{match}}$ such that 1) for all $1 \le j \le i$, $\delta_{\text{match}}(\etplt_j) = \edit_j$ and $\delta_{\text{match}}(\tplt_{i+1}^{\mathsf{pre}}) = \version_i$, and 2) the hole mappings in $\delta_{\text{match}}$ satisfy the equality relations in $\tmprel$. 
Note that, the AST to be modified in $\version_{i}$ is not known to us in real scenario.
As we evaluate the performance of a learned edit sequence pattern in our training data, we do not provide the accurate AST to be modified of $\version_{i}$ but let our matching algorithm enumerate all possible ASTs constrained by the cursor location.

To predict the $(i+1)$th edit, we need to construct a substitution $\delta_{\mathsf{pred}}$ from $\delta_{\mathsf{match}}$ and $\tmprel$ to substitute holes in $\etplt_{i+1}^{\mathsf{post}}$.
\begin{align*}
    \delta_{\mathsf{pred}} = \{\hole_1 \mapsto \delta_{\mathsf{match}}(\hole_2) \mid &(\hole_1, \hole_2) \in \tmprel \wedge \hole_1 \in dom(\tplt_{i+1}^{\mathsf{post}}) \wedge \\
    & \hole_2 \in dom(\delta_{\mathsf{match}})\},
\end{align*}
where $dom(\tplt_{i+1}^{\mathsf{post}})$ represents the set of holes in template $\tplt_{i+1}$, and $dom(\delta)$ is the domain of the substitution $\delta$.
If $\hole \notin dom(\delta_{\mathsf{pred}})$, we say the hole $\hole$ is \textit{unbounded} by $\delta_{\mathsf{pred}}$, otherwise, we say $\hole$ is \textit{bounded}. 
If all holes in $\etplt_{i+1}^{\mathsf{post}}$ are bounded by $\delta_{\mathsf{pred}}$, we can predict the version $\hat{\version}_{i+1}$ as $\delta_{\mathsf{pred}}(\tplt_{i+1}^{\mathsf{post}})$.

\begin{example}
Considering the template sequence $\tplt_1, \tplt_2$, the temporal information $\tmprel$, and the substitution $\delta_1$ in the previous examples, we can find a unique substitution $\delta$,
\[\delta_{\text{match}} = \delta_1 \cup \{\hole_{8} \mapsto \varnothing\},\]
such that we can recover $\edit_1 = \version_0 \to \version_3$ from $\tplt_1$ and the previous version of $\edit_2$ from $\tplt_2^{\mathsf{pre}}$ using $\delta_{\text{match}}$.
$\delta_{\text{match}}$ also satisfy $\tmprel$ because $\hole_{1} = \hole_{3} \wedge \hole_{2} = \hole_{7}$.

To predict the $(i+1)$th edit, we can construct $\delta_{\mathsf{pred}}$ as,
\[\delta_{\mathsf{pred}} = \{\hole_{9} \mapsto \varnothing, \hole_{10} \mapsto \textit{str}\}\]
Unfortunately, $\hole_{11}$ is unbounded, so we cannot use $\delta_{\mathsf{pred}}$ to predict the version $\version_4$.
However, we mitigate this by introducing a new relation $\tmprel_{\mathsf{lower}}$, which captures the string transformation that modifies the first character to the lower case.
In this example, $(\hole_{11}, \hole_{5}) \in \tmprel_{\mathsf{lower}}$ because the code substituting $\hole_{11}$ is equal to the code substituting $\hole_{5}$ and then modifying the first character to the lower case.
Using $\tmprel$ and $\tmprel_{\mathsf{lower}}$, we have
\[\delta_{\mathsf{pred}} = \{\hole_{9} \mapsto \varnothing, \hole_{10} \mapsto \textit{str}, \hole_{11} \mapsto \textit{id}\},\]
and we can see $\delta_{\mathsf{pred}}(\tplt_{i+1}^{\mathsf{post}}) = \version_4$.
\end{example}
}

% \begin{figure}
% {\footnotesize
% \begin{lstlisting}[language=diff]
% class Comms {
% // Edit 1
% -  void Write(Stream s, byte[] bs, bool flush) { ... }
% +  void Write(Stream s, byte[] bs) { ... }
% }
% void Main() {
% // Edit 2
% -    Comms.Write(stream, bytes, f);}
% +    Comms.Write(stream, bytes);
% // Edit 3
% -    Comms.Write(stream, resultBytes, f);
% +    Comms.Write(stream, resultBytes);
% }
% \end{lstlisting}
%   \vspace{-5ex}
% }
% \caption{Delete Child Edits}
%   \vspace{-4ex}
% \label{fig:del-param-code}
% \end{figure}

% \begin{example}\label{ex:edits}
%   % Added comment about marking each line with + and -
%   Consider the edits in Figure~\ref{fig:del-param-code}.
%   %
%   % The initial version contains only the lines in red (marked with $-$) and each
%   % edit replaces one red line with the corresponding green line (marked with $+$).
%   %
%   The edit $\edit_2$ is
%   $\DeleteChild(\smcode{(stream, bytes, f)}, \smcode{f}, 2)$.
%   %
%   Here, we use code fragments to refer to the equivalent ASTs.
%   %
%   Edits~$\edit_2$ and $\edit_3$ satisfy the edit pattern $\absEdit_{\mathsf{arg}} =
%   \mathsf{DelArg}(\mathsf{method}\gets\smcode{Write}, \smcode{param}\gets\smcode{flush})$.
%   %
%   In full, $\absEdit_{\mathsf{arg}} = \DeleteChild[\pred]$ where
%   $\pred$ is $
%   \parent\mathsf{.Kind} = \mathsf{ArgList} \land
%   \parent\mathsf{.Method} = \smcode{Write} \land
%   i = \parent\mathsf{.Params.Index(\smcode{flush})}$.
%   %
%   Generally, $\absEdit_{\mathsf{arg}}$ represents argument deletions
%   corresponding to the parameter \smcode{flush} in a call to \smcode{Write}.
%   %
%   The edit sequences $\edit_1\edit_2\edit_3$ and $\edit_2\edit_3\edit_1$
%   represent two ways of achieving the same logical edit of
%   deleting \smcode{flush} and corresponding arguments, but in different orders.
%   %
%   We have $\edit_1\edit_2\edit_3 \models \absEdit_\mathsf{param}
%   \absEdit_\mathsf{arg}^*$ and
%   $\edit_2\edit_3\edit_1 \models \absEdit_\mathsf{arg}^*\absEdit_\mathsf{param} $, where
%   $\absEdit_\mathsf{param} = \mathsf{DelParam}(\smcode{Write}, \smcode{flush})$.
%   %
%   \qed
% \end{example}


% \noindent\textbf{Temporal Edit Patterns.}
% %
% Intuitively, a temporal edit pattern is a regular expression style
% description that represents multiple edit sequence patterns for the same task.
% %
% Formally, a \emph{temporal edit pattern} $\SeqPat$ is one of:
% \begin{inparaenum}[(a)]
%   \item an edit pattern $\absEdit$,
%   \item a concatenation $\SeqPat_1 \cdot \SeqPat_2$,
%   \item a Kleene star $\SeqPat_1^*$, or
%   \item an alternation $\SeqPat_1 \mathbin{\mid} \SeqPat_2$.
%   % \item a unordered sequence $\UnorderedSeq{\SeqPat_1, \ldots, \SeqPat_n}$.
% \end{inparaenum}
% %
% Concatenation, Kleene star, and alternation have their usual meanings as in
% standard regular expressions.
% %
% \ignore{
% The unordered sequence $\UnorderedSeq{\SeqPat_1, \ldots,
% \SeqPat_n}$ states that the edit sequence pattern must match some
% permutation of $\SeqPat_1 \ldots \SeqPat_n$, i.e.,
% $\absEdit_0\ldots\absEdit_m \models \UnorderedSeq{\SeqPat_1, \ldots,
% \SeqPat_n}$ if and only if, $\absEdit_0\ldots\absEdit_m$ matches
% $\SeqPat_{i_1}\cdot\ldots\cdot\SeqPat_{i_n}$ where $i_1,\ldots, i_n$ is a
% permutation of $1, \ldots, n$.
% }
% We use the shorthand $\UnorderedSeq{\SeqPat_1, \ldots,
% \SeqPat_n}$ to denote the alternation between all permutations of
% $\SeqPat_i$.


% \begin{example}
%   In Example~\ref{ex:edits}, we saw the deletion of a parameter and
%   corresponding arguments can performed through the edit sequence patterns
%   $\absEdit_\mathsf{param}\absEdit_\mathsf{arg}\absEdit_\mathsf{arg}$ and
%   $\absEdit_\mathsf{arg}\absEdit_\mathsf{arg}\absEdit_\mathsf{param}$.
%   % where
%   % $\absEdit_\mathsf{arg} = \mathsf{DelArg}(\mathsf{m}, \mathsf{pN})$ and
%   % $\absEdit_\mathsf{param} = \mathsf{DelParam}(\mathsf{m}, \mathsf{pN})$.
%   %
%   % Several temporal edit patterns that match one or both of these edit sequence patterns.
%   %  
%   Temporal edit patterns $\SeqPat_1 =
%   \absEdit_\mathsf{param}\absEdit_\mathsf{arg}^*$ and $\SeqPat_2 =
%   \absEdit_\mathsf{arg}^*\absEdit_\mathsf{param}$ match only
%   $\absEdit_\mathsf{param}\absEdit_\mathsf{arg}\absEdit_\mathsf{arg}$ and
%   $\absEdit_\mathsf{arg}\absEdit_\mathsf{arg}\absEdit_\mathsf{param}$,
%   respectively.
%   %
%   We can further generalize $\SeqPat_1$ and $\SeqPat_2$,
%   combining both sequences as
%   $\SeqPat_1 \mathbin{\mid} \SeqPat_2$.
%   %
%   This combination can also be written using the unordered sequencing operator
%   as $\UnorderedSeq{\absEdit_\mathsf{param}, \absEdit_\mathsf{arg}^*}$.
%   \qed
% \end{example}

% \mohammad{feeling a bit of terminology overload: edits, edit sequences, edit pattern, edit sequence pattern, temporal edit pattern. Not sure if its better to  cut to the chase quickly by  formally defining the ultimate notion of temporal edit pattern that we are interested in a CFG-style definition in a figure, and then explaining it in the text}

% of similar edits using edit distance between edit embeddings~\cite{Jiang:Deckard}. \todo{if we only use $d=0$ in the Dcap, do we need to define our embedding?} \ameya{TODO}
%

% \begin{example}
%   \label{ex:generality}
%   Consider the edits $\edit_1$, $\edit_2$, and $\edit_3$
%   corresponding to adding \smcode{public int Count \{ get; \}},
%   \smcode{public int Threshold} \smcode{\{ get;set; \}}, and
%   \smcode{int size = examples.Length}.
%   %
%   Our hierarchical clustering procedure produces clusters as depicted
%   in Figure~\ref{fig:clusters}.
%   %
%   Depending on scenario, we consider $\edit_1$ under different levels
%   of generality.
%   %
%   \begin{inparaenum}[(a)]
%       \item In a copy-paste-rename sequence (see Figure~\ref{fig:copy-paste-pattern}),
%         the label of the node copy-pasted is irrelevant, and
%         we group $\edit_1$, $\edit_2$, and $\edit_3$ as ``insert child'' (cluster $\Cluster_0$). 
%         %
%       \item When adding and initializing a property,
%         $\edit_1$ and $\edit_2$ can be grouped as ``insert property''
%         (cluster $\Cluster_1$), but not with  $\edit_3$. %
%       \item In the scenario where a get property is added and used in a 
%         client class, $\edit_1$ is considered as
%         ``insert get property'' (cluster $\Cluster_4$)
%         and is distinct from both $\edit_2$ and $\edit_3$.
%   \end{inparaenum}
%   %
%   The hierarchical clustering procedure generates each of the ``insert child'',
%   ``insert property'', and ``insert get only property'' clusters, with
%   $\edit_1$ belonging to each of them.
%   %
%   Given such clusters, in the \emph{Generating Temporal Edit Patterns}
%   paragraph below, we explain how to connect the clusters at different granularities into
%   % into edit sequence patterns. and  subsequently
%   temporal edit patterns that represent the different
%   scenarios above.
%   \ignore{
%   \gustavo{this paragraph felt a little bit magical. Maybe we should say something like: in section X we will explain how we can mine relevant temporal edit patterns at all these levels of generalization}
%   }
%   %
%   \qed
% \end{example}

% \noindent\emph{Edit embeddings.}
% % We embed edits into Euclidean space using a sequence of embeddings
% % that capture increasing amount of information from the edits.
% %
% Our embeddings are based on the one presented in~\cite{Jiang:Deckard}.
% %
% For each AST node $\ASTnode$, the \emph{$d$-cap (resp. $d$-context)} of
% $\ASTnode$ (see~\cite{Nguyen2013,Evans2009}) is the set of all descendants (resp. ancestors)
% with distance $< d$.
% %
% For example, $2$-cap and $2$-context contains the $\ASTnode$ and its direct
% children, and $\ASTnode$ and its parent, respectively.

% Let $\mathsf{Labels}$ be the set of all possible AST node labels.
% %
% We define $\mathsf{S}(\ASTnodes)$ as the vector where
% $\mathsf{S}(\ASTnodes)[i]$ is the count of nodes
% with label $\mathsf{Labels}[i]$ in $\ASTnodes$.
% %
% We define the depth $d$ embedding $\embed_d(\edit)$ of an edit as:
% \[{\scriptsize
%     \begin{array}{l}
%       \:\:\:\mathsf{S}(\mathsf{DCap}(\mathsf{child})) + \mathsf{S}(\mathsf{DContext}(\mathsf{child})) 
%         \text{~~~~~~~~~~~~~~~\textbf{if $\edit = \mathsf{InsertChild}(\mathsf{parent}, \mathsf{child}, i)$}} \\
%       {-\mathsf{S}(\mathsf{DCap}(\mathsf{child}))} + \mathsf{S}(\mathsf{DContext}(\mathsf{child}))
%         \text{\textbf{~~~~~~~~~~~~~~~if $\edit = \mathsf{DeleteChild}(\mathsf{parent}, \mathsf{child}, i)$}} \\
%       \:\:\:\mathsf{S}(\mathsf{DCap}(\mathsf{new})) - \mathsf{S}(\mathsf{DCap}(\mathsf{old})) + \mathsf{S}(\mathsf{DContext}(\mathsf{new})) 
%         \text{\textbf{~~~~~~~~if $\edit = \mathsf{Update}(\mathsf{old}, \mathsf{new})$}} \\
%     \end{array}
% }\]
% %
% \ignore{
% \ashish{Is the above correct? DeleteChild should have both terms negative, and Update should not have a "Context" term.}
% Note that increasing $d$ increases the amount of information that is
% extracted from the edit into the embedding.
% \ameya{The above is correct. I have not considered the Context of delete negative because those AST nodes were not removed. Also the updates needs the context.}
% %
% }
% The function \textsc{HierarchicalClustering}
% differs from 
% % produces clusters from the set of input edits.
% %
% % Compared to
% standard algorithms in using
% different distance functions at each depth.


% \begin{figure}
%   \small
%   \tikzset{
%     cluster/.style = {draw, rounded corners, minimum width=1.5cm, minimum height=0.75cm},
%     hidden/.style = {draw, dotted, minimum height=0.5cm, minimum width=1cm}
%   }
%   \scalebox{0.75}{
%   \begin{tikzpicture}
%     \node[cluster]                             (insert)             {$\Cluster_0$: $\InsertChild$};

%     \node[cluster, xshift=-3.0cm, yshift=-1.0cm] (add prop)           {$\Cluster_1$: Insert Property};
%     \node[cluster, xshift=+0.0cm, yshift=-1.0cm] (add stmt)           {$\Cluster_2$: Insert Statement};
%     \node[cluster, xshift=+3.0cm, yshift=-1.0cm] (add param)          {$\Cluster_3$: Insert Parameter};

%     \node[cluster, xshift=-6.4cm, yshift=-2.5cm]   (add get prop)       {\tabular{c}$\Cluster_4$: Insert\\Get-Only\\Property\endtabular};
%     \node[cluster, xshift=-4.1cm, yshift=-2.5cm]   (add get set prop)   {\tabular{c}$\Cluster_5$: Insert\\Get-Set\\Property\endtabular};
%     \node[cluster, xshift=-2.0cm, yshift=-2.5cm]   (add get init prop)  {\tabular{c}$\Cluster_6$: Insert\\Get-Init\\Property\endtabular};

%     \node[hidden,  xshift=-0.5cm, yshift=-2.5cm]                              (add stmt child 1)     {};
%     \node[hidden,  xshift=+1.0cm, yshift=-2.5cm]                              (add stmt child 2)     {};

%     \node[hidden,  xshift=+2.5cm, yshift=-2.5cm]                              (add param child 1)     {};
%     \node[hidden,  xshift=+4.0cm, yshift=-2.5cm]                              (add param child 2)     {};

%     \draw[->]           (insert)    -- (add prop);
%     \draw[->]           (insert)    -- (add stmt);
%     \draw[->]           (insert)    -- (add param);
%     \draw[->]           (add prop)  -- (add get prop);
%     \draw[->]           (add prop)  -- (add get set prop);
%     \draw[->]           (add prop)  -- (add get init prop);
%     \draw[->, dotted]   (add stmt)  -- (add stmt child 1);
%     \draw[->, dotted]   (add stmt)  -- (add stmt child 2);
%     \draw[->, dotted]   (add param) -- (add param child 1);
%     \draw[->, dotted]   (add param) -- (add param child 2);
%   \end{tikzpicture}
%   }
%   \vspace{-4ex}
%   \caption{
%     Fragment of Hierarchical cluster structure produced
%     by procedure \textsc{HierarchicalClustering}.
%     \ameya{Should we update this figure? Since we use single level of hierarchy now}
%     \yh{Maybe we will just remove this figure.}
%   }
%   \label{fig:clusters}
%   \vspace{-4ex}
% \end{figure}

% \begin{example}
%   \label{ex:cluster-to-pattern}
%   Figure~\ref{fig:clusters} shows a part of the hierarchical clusters
%   produced by the procedure \textsc{HierarchicalClustering}.
%   %
%   As shown in Example~\ref{ex:generality}, the clusters account for the
%   generality problem depicted in Section~\ref{sec:motivating-example}.
%   %
%   We obtain clusters $\Cluster_1$, $\Cluster_2$ and $\Cluster_3$
%   by performing unsupervised clustering on $\Cluster_0$ using the distance
%   function $\embed_1$.
%   %
%   Embedding $\embed_1$ only encodes the label of the AST node,
%   e.g., $\mathsf{Statement}$, $\mathsf{Property}$, etc.
%   %
%   The distance between all edits on the same label is $0$,
%   and for different labels is non-zero.
%   %
%   Hence, we get clusters corresponding to insertion of each kind of AST node.

%   At depth $2$, the edits in $\Cluster_1$ are clustered using $\embed_2$, which
%   %
%   encodes information about the inserted property's:
%   \begin{inparaenum}[(a)]
%     \item parent (here, always a $\mathsf{ClassBody}$), and
%     \item direct children (e.g., $\mathsf{GetAccessor}$ and
%         $\mathsf{SetAccessor}$).
%   \end{inparaenum} 
%   %
%   Therefore, $\embed_2$ incorporates accessor information and we obtain the clusters
%   $\Cluster_4$ insert get-only property, 
%   $\Cluster_5$ insert get-set property, and
%   $\Cluster_6$ insert get-init property.
%   \qed
% \end{example}

% In theory, we may produce clusters of any arbitrary collection
% of edits, while in practice, as shown in Example~\ref{ex:cluster-to-pattern},
% they correspond to clear edit patterns.
% %
% Our implementation of \technique can automatically label these
% clusters with corresponding edit patterns.

\ignore{
Now we combine the resulting edit sequence patterns into temporal edit patterns.
%
The combination is done by repeated application of two heuristic rules:
%
\begin{inparaenum}[(a)]
  \item Given patterns $\absEdit_0\ldots\absEdit_n\absEdit_{n+1}^{p}$
    and $\absEdit_0\ldots\absEdit_n\absEdit_{n+1}^{q}$ for $p \neq q$, we generalize
    them into $\absEdit_0\ldots\absEdit_n \cdot \absEdit_{n+1}^*$.
  \item Given temporal edit like patterns for all permutations of $\absEdit_1$,
    \ldots $\absEdit_n$, then we generalize them into
    $\UnorderedSeq{\absEdit_1, \ldots, \absEdit_n}$.
\end{inparaenum}
%
These rules while simple, suffice in practice.
%
These rules can be augmented with a manual summarization step to further 
generalize the patterns if necessary.
}


\ignore{

\subsection{Guided Exploration}
\label{sec:querying}

Given the quotient graph summary from the previous
Section~\ref{sec:clustering}, we present a mechanism where a user and the
system can explore the space of temporal edit patterns to discover insights
about the input development sessions.
%
An edit path in the quotient graph is a sequence $\Cluster_0\ldots\Cluster_n$
where each cluster is connected to the next with a sequencing edge, i.e.,
$\forall i. \Cluster_i \to_\seq \Cluster_{i+1}$.
%
For each edit path, a concrete edit path is given by $\edit_0 \ldots \edit_n$
such that $\forall i. \edit_i \in \Cluster_i$ and $\edit_0\ldots\edit_n$ is a
sequence of contiguous edits that occur in some input development session.
%

The exploration component of \technique accepts $2$ distinct types of inputs:
\begin{itemize}
  \item \emph{Statistical query.} These are bounds on the concrete paths
    corresponding to the edit path.
    Currently, we allow constraints on the number of concrete paths
    corresponding to the edit path, as well as on the number of unique
    sessions and developers that correspond to the concrete paths.
  \item \emph{Edit example query.} These queries return an edit path
    consisting of a single cluster to which the concrete edit example belongs.
\ignore{
\item \emph{Edit set example query.} These queries return all edit paths
    which are composed of clusters that match any edit in the example edit
    set.
}
\end{itemize}
%
Exploration in \technique happens through two operations that modify edit
paths.
%
\begin{itemize} 
  \item \emph{Extend.} Given a path $\Cluster_1\ldots\Cluster_n$,
    the extend operation produces either
    \begin{inparaenum}[(a)]
      \item the path $\Cluster_0\ldots\Cluster_n$ where
        $\Cluster_0 \to_\seq \Cluster_1$, or
      \item the path $\Cluster_1 \ldots \Cluster_n \Cluster_{n+1}$ where
        $\Cluster_n \to_\seq \Cluster_{n+1}$.
    \end{inparaenum}
    This operation adds either a prior or a subsequent edit cluster to the
    path.
  \item \emph{Fragment.} Given a path
    $\Cluster_1\ldots\Cluster_i\ldots\Cluster_n$, the fragment operation
    replaces $\Cluster_i$ at depth $d$ with a sequence
    $\Cluster_{i_1}\ldots\Cluster_{i_m}$ where each $\Cluster_{i_k}$ is a
    cluster at depth $d+1$.
    %
    In addition, we ensure that $\Cluster_i$ subsumes $\Cluster_{i_j}$ for
    all $j$, and that there exist edits in each $\Cluster_{i_j}$ whose
    composition produces an edit from $\Cluster_i$.
    %
    Optionally, \technique can produce all possible fragmentations along with
    their frequencies.
    \ignore{
    In addition, we have the following conditions:
    \begin{inparaenum}[(a)]
      \item For every $\Cluster_{i_k}$ there exists a subsumption edge
        $\Cluster_i \to_\sub^q \Cluster_{i_k}$,
      \item $\not \exists \Cluster. \Cluster_i \to_\sub \Cluster \land
        \Cluster \to_\seq \Cluster_{i_1}$, and
      \item $\not \exists \Cluster. \Cluster_i \to_\sub \Cluster \land
        \Cluster_{i_k} \to_\seq \Cluster$.
        %
        Intuitively, the operation refines edit cluster $\Cluster_i$ to a
        finer level of granularity.
    \end{inparaenum}
    }
\end{itemize} 
%
In the following example, we demonstrate how an IDE designer may explore the
query and action tools.

\begin{example}[Interacting with \technique.]
  Let us examine in detail a sample interaction with \technique.
  %
  Suppose an IDE designer want's to examine the add and initialize property
  task from Section~\ref{sec:motivating-example}.
  %
  
  First, the designer provides an example of the whole change they want to
  examine.
  %
  Suppose they provide the example $\version_0 \to \version_5$ from
  Figure~\ref{fig:dev-session}.
  %
  Now, \technique produces the cluster with the edits most similar to
  $\version_0 \to \version_5$ ($\Cluster_0$ from Figure~\ref{fig:quotient_graph}).
  %
  \arsays{This?
  The designer can now examine the other edits in $\Cluster_0$ to ensure that
  they are similar to the add and initialize property example edit at hand.
  }
  %
  Further, at this point, the developer may rename the cluster $\Cluster_0$ to
  aid future exploration.

  The designer is interested in the most frequent sub-edit patterns that are
  performed during this edit pattern.
  %
  \technique can return clusters that are subsumed by $\Cluster_0$ by following
  the subsumption edges in the quotient graph.
  %
  As expected, the subsumed clusters with the most number of edits are the
  clusters corresponding to adding a property $\Cluster_1$, adding a constructor
  parameter $\Cluster_2$, and adding an assignment $\Cluster_3$.
  %

  Now, the designed is interested in what manner developers perform the main
  edit pattern, i.e., in which order are the sub-tasks performed.
  %
  \technique can fragment $\Cluster_0$ and produce multiple edit pattern
  sequences that witness the sub-cluster.
  %
  While Figure~\ref{fig:quotient_graph} only depicts the edges and path
  $\Cluster_1 \to_\seq \Cluster_2 \to_\seq \Cluster_3$, in our experiments,
  we found paths for all permutations of $\Cluster_1$, $\Cluster_2$, and
  $\Cluster_3$.
  %
  This indicates that multiple developers over multiple times performed this
  three sub-patterns in all orders.
  %
  The designer now has the insight about the temporal order of actions
  followed by developers: in this case, the authors of this paper were
  surprised by the orders in which the assignment was added first.

  At this point, \technique can summarize the multiple edit sequence patterns
  into a single temporal pattern.
  %
  In this case, the temporal pattern is equivalent to
  $\UnorderedSeq{\Cluster_1, \Cluster_2, \Cluster_3}$.
  %
  This temporal edit pattern may now be stored for future investigation or
  tool building.
  %
  For simple cases such as these, \technique is able to generate the temporal
  edit pattern automatically.
  %
  For more complex instances, it might need help from the designer to build
  the temporal edit pattern.
  %
  \qed
\end{example}
}

\begin{inparaenum}[(a)]
  \item $\edit$ \emph{subsumes} $\edit'$ if $i \leq k < \ell \leq j$ and $\edit
    \neq \edit'$, and
  \item $\edit'$ \emph{sequentially follows} $\edit$ if $i < j = k < l$.
\end{inparaenum}

\begin{algorithm}
  \small
  \begin{algorithmic}[1]
    \Require Development sessions $\mathsf{Sessions}$, Connection strength $n$
    \Ensure Sketches of edit sequence pattern $\mathsf{Sketches}$
    \Function{ClusterEdit}{$\edits$, $\mathsf{threshold}$}
    % \State $\Clusters_0 \gets \{ \mathsf{Inserts}(\edits), \mathsf{Deletes}(\edits), \mathsf{Updates}(\edits)\}$
    % \State $d \gets 0$
    % \While {$\Clusters_d \neq \emptyset$}
    %   \State $d \gets d + 1$
    %   \State $\Clusters_d \gets
    %     \bigcup \{ \mathsf{Clustering}(\Cluster, \embed_d) \mid
    %     \Cluster \in \Cluster_d \land |\Cluster| > 1 \}
    %   $
    % \EndWhile
    % \State \Return $\bigcup_d \Clusters_d$
    \State $\mathsf{Partitions} \gets \{ \mathsf{Inserts}(\edits), \mathsf{Deletes}(\edits), \mathsf{Updates}(\edits)\}$
    \State \Return $\bigcup_{\mathsf{p} \in \mathsf{Partitions}} \mathsf{ParitionByASTKind}(\mathsf{p})$
    \EndFunction

    \Function{BuildEditGraph}{$\mathsf{edits}$}
    \State $\edits \gets$ \Call{Prune}{$\edits$}
    \State $\Esub \gets \{~~\edit \to \edit' \mid \exists~\edit,\edit' \in \mathsf{edits}.$
        $\mathsf{SameSession}(\edit,\edit') \land$
        $\hphantom{.}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\edit \to_\sub \edit'~~\}$
    \State $\Eseq \gets \{~~\edit \to \edit' \mid \exists~\edit,\edit' \in \mathsf{edits}.$
        $\mathsf{SameSession}(\edit,\edit') \land$
        $\hphantom{.}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\edit \to_\seq \edit'~~\}$
    \State $\mathsf{EditGraph} \gets \langle V = \edits, \Esub, \Eseq \rangle$
    \EndFunction

    \Function{Quotient}{$\langle V, \Esub, \Eseq\rangle$, $\mathsf{CS}$, $n$}
    \State $V^q \gets \mathsf{CS}$
    \State \Comment{Below, $\exists^n$ stands for there exist $n$ distinct}
    \State $\Esub^q \!\gets\! \{ \mathsf{C} \to \mathsf{C}' \!
        \mid \! \mathsf{C},\mathsf{C'} \!\in \mathsf{CS} \land
        \exists^n \edit \in \mathsf{C}, \edit' \!\in \mathsf{C}'. \edit \!\to\! \edit' \!\in \Esub
      \}$
    \State $\Eseq^q \!\gets\! \{ \mathsf{C} \to \mathsf{C}' \!
        \mid \! \mathsf{C},\mathsf{C'} \!\in \mathsf{CS} \land
        \exists^n \edit \in \mathsf{C}, \edit' \!\in \mathsf{C}'. \edit \!\to\! \edit' \!\in \Eseq
      \}$
    \State \Return $\langle V^q, \Esub^q, \Eseq^q \rangle$
    \EndFunction

    \Function{MineTemporalEditPatterns}{$\mathsf{Sessions}$, $\mathsf{threshold}$}
    \State $\edits \gets \bigcup \{ \Edits(\Session) \mid \Session \in \mathsf{Sessions} \} $
    \State $\mathsf{EditGraph} \gets$ \Call{BuildEditGraph}{$\mathsf{edits}$} 
    \State $\mathsf{Partitions} \gets$ \Call{PartitionEdits}{$\mathsf{edits}$, $\mathsf{threshold}$} 
    \State $\mathsf{TemporalSummary} \gets$ \Call{Quotient}{$\EditGraph$,$\mathsf{Partitions}$, $n$}
    \State $\mathsf{Sketches} \gets \Call{FrequentPatterns}{\mathsf{TemporalSummary}}$
    \State \Return $\mathsf{Sketches}$
    \EndFunction
  \end{algorithmic}
  \caption{The procedure of synthesizing sketches of edit sequence patterns}
  \label{algo}
\end{algorithm}

Starting with the set of all filtered edits as described above, the function \textsc{PartitionEdits} in Algorithm~\ref{algo} simply partitions based on the \textit{kind} of the AST node (e.g. \textit{method invocation} or \textit{indentifier}) which is affected by the edit and the \textit{kind} of edit applied (i.e. \textit{Insert}, \textit{Update} or \textit{Delete}).
For instance, \textsc{PartitionEdits} will produces partitions like \textit{Insert-Property}, \textit{Insert-Local Variable}, \textit{Delete-argument} or \textit{Update-Identifer}.

\begin{figure}
  \vspace{-1ex}
  \small
  \tikzset{
    cluster/.style = {draw, rounded corners, minimum width=1.5cm, minimum height=0.75cm},
    seq/.style = {->, blue, thick, dashed},
    sub/.style = {->, red, thick, dotted}
  }
  \scalebox{0.7}{
  \begin{tikzpicture}
    \node[cluster] (prop param ass) {\tabular{c}$\Cluster_0$: Add + Init Prop\\(e.g., $\version_0 \to \version_5$)\endtabular};

    \node[cluster, xshift=-3cm, yshift=-1.5cm] (prop)          {\tabular{c}$\Cluster_1$: Add Get-Set Prop\\(e.g., $\version_0 \to \version_3$)\endtabular};
    \node[cluster, xshift=+0cm, yshift=-1.5cm] (param)          {\tabular{c}$\Cluster_2$: Add Param\\(e.g., $\version_3 \to \version_4$)\endtabular};
    \node[cluster, xshift=+3cm, yshift=-1.5cm] (ass)          {\tabular{c}$\Cluster_3$: Add Assign\\(e.g., $\version_4 \to \version_5$)\endtabular};

    \node[cluster, xshift=-6cm, yshift=-3cm] (get prop)          {\tabular{c}$\Cluster_4$: Add Get Prop\\(e.g., $\version_0 \to \version_2$)\endtabular};
    \node[cluster, xshift=-2cm, yshift=-3cm] (set prop)          {\tabular{c}$\Cluster_5$: Make Prop Settable\\(e.g., $\version_2 \to \version_3$)\endtabular};

    \draw[seq] (prop) -- (param);
    \draw[seq] (param) -- (ass);

    \draw[sub] (prop param ass) -- (prop);
    \draw[sub] (prop param ass) -- (param);
    \draw[sub] (prop param ass) -- (ass);

    \draw[sub] (prop) -- (get prop);
    \draw[sub] (prop) -- (set prop);

    \draw[seq] (get prop) -- (set prop);

    \draw[seq] (set prop) -- (param);
  \end{tikzpicture}
  }
  \vspace{-2ex}
  \caption{
    Temporal edit summary for the add and initialize
    property scenario.
    %
    Red dotted edges and blue dashed edges represent subsumption and
    sequencing, respectively.
  }
  \label{fig:quotient_graph}
  \vspace{-4ex}
\end{figure}

\ameya{If we redraw the Fig 5 such that C1 and C4 are merged, we won't be able to show that our partitioning allows us to "mix-n-match" edit partitions to produce edit sequences at varying granularity. My suggestion would be to remove this Fig 5 and related text.}
\textcolor{red}{\begin{example}
  Figure~\ref{fig:quotient_graph} illustrates the quotient graph for the
  scenario from Figure~\ref{fig:dev-session}.
  %
  The add and initialize property cluster $\Cluster_0$ subsumes 
  the add property $\Cluster_1$, add parameter $\Cluster_2$, and
  add assignment $\Cluster_3$ clusters, 
  %
  breaking up $\Cluster_0$ into $3$ separate smaller steps.
  %
  The add property cluster is again sub-divided into two clusters
  (add a get-only property $\Cluster_4$ and make a property settable $\Cluster_5$).
  %
  Note the sequencing edge between $\Cluster_5$ and $\Cluster_2$.
  %
  This cross connection between different depths allows us
  \emph{``mix-and-match''} granularity levels in the same edit sequence
  pattern.
  %
  We can potentially generate two different temporal
  edit patterns, one related to ``make property settable'' and ``add parameter''
  and another related to ``add get-set prop'' and ``add parameter''; that is, we 
  can treat $\version_0 \to \version_3$ both atomically and as a 
  combination of $\version_0 \to \version_2$ and $\version_2 \to \version_3$.
\end{example}
}
The quotient graph summarizes information at multiple levels of
\begin{inparaenum}[(a)]
  \item generalization, as each edit is a part of multiple partitions; and
  \item granularity, as it contains partitions corresponding to both coarse
    grained and fine-grained edits with subsumption edges between them.
\end{inparaenum}
%

\ameya{Remove}
\textcolor{red}{In the manual step, the user validates these cluster expression and converts
them into temporal edit patterns by replacing clusters with equivalent
edit patterns.
%
The need for validation is due to sketches lacking parameter constraints.
%
For example, in 
$\mathsf{DelParam}(\mathsf{method}, \mathsf{paramName})
\cdot \mathsf{DelArg}(\mathsf{method}, \mathsf{paramName})$,
we want the method and parameter name
to be shared across the edit patterns.
%
However, in the cluster path, this constraint might not be ensured.
%
As in~\cite{Negara:ICSE:MiningEdits,Nguyen:CPatMiner,revisar}, we rely on the user to ensure that at least one
concrete edit sequence corresponding to the cluster path satisfies 
this constraint.
%
Then, the user annotates each cluster with the equivalent edit pattern.}

Based on a user-provided upper bound on the length, we generate paths
in the quotient graph.
%
To generate these, \technique first starts by considering all length $1$ paths, i.e.,
a single partiton.
%
Iteratively, we generate new paths by extending the
edit sequence patterns $\Partition_1\ldots\Partition_n$ by appending $\Partition_{n+1}$ if
\begin{inparaenum}
\item $n + 1$ is less that the length bound, 
\item there exists at least one concrete edit sequence in an input session that
    corresponds to the path $\Partition_1\ldots\Partition_{n+1}$, and
\item there exists a partition $\Partition$ such that $\forall 1 \leq i \leq n + 1.
    \Partition \to_\sub \Partition_i$.
\end{inparaenum}
%
At this point, we combine the partition paths into cluster expressions, which
are akin temporal edit expressions, but with edit patterns replaced with partitions.
%
This combination is done heuristically, by introducing Kleene stars on single
partitions based on the existence of self-edges in the quotient graphs, and by
replacing cluster paths corresponding to all permutations of a set of partitions
with the unordered sequence operator.

We first select a list of edit sequence patterns using a greedy algorithm by evaluating their performance on all edit sequences we collected in Section~\ref{sec: marjor_step_1}.
We further rank the selected list of edit sequence patterns by evaluating their performance on the development sessions as a simulation in the real-world scenario. 

% We want to represent each edit sequence pattern as a list of edit sequence patterns because of the following reasons.~\yh{reasons for selection in short: overcome noise, hierarchical structure}
% First, the mined edit sequences are noisy, meaning the most general edit sequence patterns (near the root of a dendrogram) would be too general and possibly generate more false positives, while the most specific edit sequence patterns (near the leaves of a dendrogram) would be too specific and possibly generate more false negatives.
% Second, the dendrogram learns a hierarchical structure of each edit sequence pattern such that different nodes in the dendrogram can be interpreted as different developer intents.~\yh{more precise word than ``intents''?}
% Furthermore, we will rank the list of edit sequence patterns because we might prefer some edit sequence patterns than others as shown in the following example.
% \begin{example}
% Our approach selects and ranks two edit sequence patterns to represent the edit sequence pattern ``Create Property'', namely, 1) ``Add public property''$\to$``Add  get''$\to$``Add private set'', and 2) ``Add any property''$\to$``Add  get''$\to$``Add set''. 
% Our approach prefers the first edit sequence pattern because it is more likely for developers to construct a public property with ``private set'' than with ``set'' in our learning dataset. 
% \end{example}

We propose a greedy covering algorithm to select edit sequence patterns using their performance on all edit sequences.
We first evaluate the performance of every edit sequence patterns over all edit sequences. 
We have defined the prediction of the next version using edit sequence patterns given a prefix of edit sequences in Section~\todo{X}.
Each edit sequence pattern will have three outcomes on an edit sequence,
\begin{inparaenum}
  \item we say the edit sequence pattern correctly predicts the edit sequence $\edit_1\ldots\edit_n$ if the edit sequence pattern correctly predict every edit $\edit_i (i>1)$,
  \item we say it mispredicts the edit sequence if the edit sequence pattern mispredicts one edit before it fails to match an edit,
  \item otherwise, we say it does not predict on the edit sequence.
\end{inparaenum}
We define the \emph{precision} of an edit sequence pattern as $\frac{\text{\#correct\_pred}}{\text{\#correct\_pred} + \text{\#mis\_pred}}$ and the \emph{contribution} of it as $\text{\#correct\_pred} - \text{\#mis\_pred}$.
The greedy covering algorithm maintains a set of selected edit sequence patterns and a set of uncovered edit sequences.
At each iteration, the algorithm selects the edit sequence pattern that have at least $\mathsf{threshold}$ precision and have the largest contribution over the uncovered edit sequences.
The algorithm runs until the set of uncovered edit sequences is empty or it cannot select a valid edit sequence pattern.

Each development session is a sequence of versions of each source file as shown in Figure~\ref{fig:dev-session}.
To evaluate each edit sequence pattern on version $\version_i$, we need to 
\begin{inparaenum}
  \item enumerate all sequences of edits ending at $\version_i$ which match a prefix of the edit sequence pattern, 
  \item predict the next version $\version_{\mathsf{pred}}$ (if there are multiple predictions given by the same edit sequence pattern, we will select the one with the shortest edit sequence), and 
  \item check whether there is a version $\version_j (j>i)$ equals $\version_{\mathsf{pred}}$. If there is, we say the edit sequence pattern correctly predict at $\version_i$, otherwise, we say it mispredicts.
\end{inparaenum}
We compute the \emph{precision of each edit sequence pattern} as $\frac{\text{\#correct\_pred}}{\text{\#correct\_pred} + \text{\#mis\_pred}}$, similarly.
And we rank the edit sequence patterns by their precision on the development sessions.
\yh{Do we want to give the following details about the efficiency of step (1)?}
In our implementation of step, we maintain a deterministic finite automaton for each edit sequence pattern and record to which state the current version matches so that we can do step (1) efficiently.


\ignore{
The building process starts with a set of edit sequences coming from the sketch of edit sequence pattern.
We generalize every edit $\edit=\vpre \to \vpost$ by replacing same sequences of ASTs appearing in both $\vpre$ and $\vpost$ with same special nodes.
This generalization helps us generalize the edit templates we learned, e.g., we will only generate two holes in the post template for ``deleting a parameter'' regardless of how many parameters in the method. \yh{we may move the remove same procedure to the definition of edits?}
If the sketch does not contain Kleene stars, all edit sequences can be regarded as edit sequence patterns without holes.
If the sketch contains Kleene stars, the length of edit sequence can be different than the length of the edit sequence pattern. 
We will then break each edit sequence into a set of edit sequences with the same length of the edit sequence pattern.
For example, for an edit sequence $a_1b_1b_2b_3$ in sketch $AB^*$, we break the edit sequence into three edit sequences $a_1b_1, a_1b_2, a_1b_3$ which have the same length of the sketch.

The building process iteratively merges two of edit sequence patterns in the set and then adds the merged edit sequence pattern into the set until the set has the only one edit sequence pattern that is the root of the dendrogram.
Next, we present how the building process merges two edit sequence patterns and how it selects two edit sequence patterns to merge.

\todo{reflect the general function relation}
We use anti-unification~\cite{refazer, getafix, onepointone} to merge two edit template sequences $\tpltseq^{\leftts}, \tpltseq^{\rightts}$ into $\tpltseq^{\parts}$ and two temporal information $\tmprel^{\leftts}, \tmprel^{\rightts}$ into $\tmprel^{\parts}$, and we define the cost using the results of anti-unification. 
Different from existing works, we need to anti-unify not only the edit templates in two edit template sequences, but also anti-unify the temporal information. 
We use the same anti-unification algorithm as \citet{onepointone} to anti-unify the edit templates.
The algorithm outputs two substitutions $\delta_\leftts$ and $\delta_\rightts$ such that $\delta_\leftts(\tpltseq^{\parts}) = \tpltseq^{\leftts}$ and $\delta_\rightts(\tpltseq^{\parts}) = \tpltseq^{\rightts}$.
We define the anti-unification of the temporal information using $\delta_\leftts$ and $\delta_\rightts$ as,
\begin{align*}
    \tmprel^{\parts} = \{(\hole_1, \hole2) \mid& \hole_1, \hole_2 \in dom(\tpltseq^{\parts}) \wedge \\
    &\delta_\leftts(\hole_1)=\delta_\leftts(\hole_2) \wedge \delta_\rightts(\hole_1)=\delta_\rightts(\hole_2) \},
\end{align*}
where $dom(\tpltseq^{\parts})$ denotes the set of all holes in template sequence $\tpltseq^{\parts}$ and $\delta(\hole_1) = \delta(\hole_2)$ means the ASTs substituting two holes are equivalent, and if $\delta(\hole_1), \delta(\hole_2) \in \holespace$, we check the equivalent using equivalence relation $\tmprel^{\leftts}$ and $\tmprel^{\rightts}$.
And we define the cost of anti-unifying two edit sequence patterns as,
\begin{small}
\begin{align*}
    &\cost(\tpltseq^{\parts}, \tmprel^{\parts}) = \frac{|\tpltseq^{\parts}| - |dom(\tpltseq^{\parts})| + \sum_{[\hole] \in dom(\tpltseq^{\parts})/ \tmprel^{\parts}}\cost(\hole)}{|\tpltseq^{\leftts}| + \tpltseq^{\rightts}|}\\
    &\cost(\hole) =  \begin{cases}
0.5, & \delta_\leftts(\hole) \in \holespace, \delta_\rightts(\hole) \in \holespace\\
|\delta_\leftts(\hole)|+0.5, & \delta_\leftts(\hole) \notin \holespace, \delta_\rightts(\hole) \in \holespace\\
|\delta_\rightts(\hole)|+0.5, & \delta_\leftts(\hole) \in \holespace, \delta_\rightts(\hole) \notin \holespace\\
|\delta_\leftts(\hole)| + |\delta_\rightts(\hole)| - 0.5, & \text{otherwise}
\end{cases},
\end{align*}
\end{small}%
where $|\tpltseq|$ is the size of all ASTs in $\tpltseq$ and $dom(\tpltseq^{\parts})/ \tmprel^{\parts}$ is the quotient set of the equivalence relation $\tmprel^{\parts}$ over all holes in $\tpltseq^{\parts}$.
Intuitively, the $\cost(\hole)$ computes the cost of all holes in the edit template sequence, while the cost of equivalent holes are only consider once by using the quotient set.
We propose an algorithm using dynamic programming to compute the anti-unification result $\tpltseq^{\parts}$ and $\tmprel^{\parts}$ while minimizing the cost. \todo{write the algorithm (in appendix)}

At every iteration, the building process will select two edit sequence patterns that have the lowest merging cost and the merged edit sequence pattern should not have any unbounded holes.
We further break ties by the size of the temporal information $\tmprel$, i.e., we prefer the one with the largest $\tmprel$.

\begin{example}
Consider two edit sequence patterns $\tpltseq^{\leftts} = \etplt_1^{\leftts}$, $\tmprel^{\leftts}$ and $\tpltseq^{\rightts} = \etplt_1^{\rightts}$, $\tmprel^{\rightts}$, where
\begin{align*}
    \etplt_1^{\leftts} = \hole_1,\ \hole_2\ \hole_3 \to \hole_4, \quad \tmprel^{\leftts} = \{(\hole_1, \hole_4)\} \\
    \etplt_1^{\rightts} = \hole_5\ \hole_6,\ \hole_7 \to \hole_8, \quad \tmprel^{\rightts} = \{(\hole_7, \hole_8)\} 
\end{align*}
Note that the edit template sequences always contain more than one edit template, we only consider one edit template in this example for simplicity. Intuitively, the first edit template represents the pattern ``delete the last parameter'' and the second edit template represents the pattern ``delete the first parameter''.
The merged edit sequence pattern generated by our anti-unification algorithm is
\begin{align*}
     \etplt_1^{\parts} &= \hole_9,\ \hole_{10}\ \hole_{11},\ \hole_{12} \to \hole_{13},\ \hole_{14} \\ 
     \tmprel^{\parts} &= \{(\hole_{9}, \hole_{13}), (\hole_{12}, \hole{14})\} 
\end{align*}
The merging cost is $\frac{0.5 + 0.5 + 0.5 + 0.5}{4 + 4} = 0.25$.
Intuitively, the merged edit sequence pattern describes the pattern that deletes a parameter at any position. 
Our algorithm will not generate the following edit sequence pattern because its cost $\frac{0.5 + 0.5 + 0.5 + 0.5 + 0.5}{4 + 4} = 0.3125$ is higher than the previous one.
\begin{align*}
     \etplt_1^{\parts} &= \hole_9,\ \hole_{10}\ \hole_{11},\ \hole_{12} \to \hole_{13} \\ 
     \tmprel^{\parts} &= \{\} 
\end{align*} 
\end{example}
}


==> feature-request.tex <==
% \newcolumntype{L}{>{\tiny}c} 
\newcolumntype{T}{>{\footnotesize}l} 
\begin{table}[htbp]
\centering
\fontsize{7pt}{8pt}\selectfont

\begin{threeparttable}
\begin{tabular}{lccc}
\toprule
\normalsize\textbf{Id} &  \normalsize\textbf{Total} & \normalsize\textbf{TP} & \normalsize\textbf{Precision} \\
\toprule
R-337986  & 2 & 2 & 1.0 \\
G-9863    & 12 & 12 & 1.0 \\
R-381288  & 14 & 14 & 1.0 \\
G-29677    & 32 & 23 & 0.72\\
G-28760    & 2 & 2 & 1.0 \\
R-481301  & 4 & 0 & 0 \\
R-479403  & 4 & 4 & 1.0 \\
G-39138     & 4 & 0 & 0 \\
G-31836     & 0 & 0 & - \\
G-28762     & 0 & 0 & - \\
G-46700     & 0 & 0 & -\\
G-19577     & 4 & 2 & 0.5 \\
\midrule

G-43016     &  31 & 20 & 0.64 \\
R-337124     & 2 & 2 & 1.0 \\
G-38011     & 2 & 2 & 1.0 \\
G-30466     &  5 & 5 & 1.0 \\
G-45198     &  0 & 0 & - \\
% \midrule
 G-30464     & 0 & 0 & -  \\
G-32538     & 0 & 0 & - \\
G-38083     &  0 & 0 & - \\
R-17501     &  - & - & - \\
R-274811     & - & - & - \\
\midrule
   &  \textbf{\totalReportedPatterns} & \textbf{\totalTPs} & \textbf{\precision }\\
\bottomrule
\end{tabular}
\caption{Precision of our technique to find specific patterns}
\label{tab:feature-requests}
\end{threeparttable}
\end{table}

==> formalism.tex <==
\section{Edit Sequence Patterns}

To precisely describe the results of our analysis, we define the concepts of
\emph{abstract edits} and \emph{edit sequence patterns}.
%
Intuitively, an abstract edit corresponds to a single type of self-contained
logical edit and an edit sequence pattern is a combination of abstract edits.
%
For example, all edits that change the name of a property in its declaration
is an abstract edit, i.e., it is a pattern of edits that recurs often.
%
All sequences of edits that consist of changing a property name and then
updating all the use locations is an edit sequence pattern.


\noindent\textbf{Parametrized Abstract Edits.}
The aim of this paper is to characterize related edits that occur
sequentially, one after another.
%
For example, a common sequence of edits is to delete a parameter from a
method declaration, and then delete the corresponding argument from a call to
the method.
%
These edits are represented by $\mathsf{DelParam}[\mathsf{method},
\mathsf{paramName}]$ and $\mathsf{DelArg}[\mathsf{method},
\mathsf{paramName}]$.
%
However, these two abstract edits independently do not represent the scenario
described above.
%
There is no constraint to enforce that the method name and the parameter name
are the same across the two abstract edits.
%
We need to encode the information flow from the first abstract edit
to the second; the values of the parameters $\mathsf{method}$ and
$\mathsf{paramName}$ should be set by the first and be consumed by the
second.
%
We formalize this notion using the notion of in parameters and out
parameters.

An formal parameter $\mathsf{p}$ of a predicate $\pred$ can either be an
\emph{in parameter} (written as $\inparam{p}$) or an \emph{out parameter}
(written as $\outparam{p}$).
%
Formally, given two valuations $\ParamVal$ and $\ParamVal'$ that map
the formal parameters of $\pred$ to their value, we say that an edit $\edit$
\emph{satisfies $\absEdit$ in the context $\ParamVal$ and returns
$\ParamVal'$} (written as $\edit \models
\{\ParamVal\}\absEdit\{\ParamVal'\}$) if:
\begin{itemize}
\item $\pred[\forall \mathsf{p}. \inparam{p} \gets
  \ParamVal(\mathsf{p})][\forall \mathsf{p}. \outparam{p} \gets
  \ParamVal'(\mathsf{p})]$ evaluates to true, i.e., substituting the in and
  out parameters by their values in $\ParamVal$ and $\ParamVal'$ should make
  $\pred$ evaluate to true; and
\item $\ParamVal'[\mathsf{p}] = \ParamVal[\mathsf{p}]$ if $\outparam{p}$ does
  not occur in $\mathsf{pred}$, i.e., the values of the parameters that are
  not set by $\mathsf{pred}$ should be the same across $\ParamVal$ and
  $\ParamVal'$.
\end{itemize}
%
We extend this definition to a sequence of edits and a sequence of abstract
edits by saying that the relation $\edit_0\ldots\edit_n \models
\{\ParamVal\}\absEdit_0\ldots\absEdit_n\{\ParamVal'\}$ holds if:
%
there exists $\ParamVal_0\ldots\ParamVal_{n+1}$ such that $\ParamVal =
\ParamVal_0$ and $\ParamVal' = \ParamVal_{n+1}$, and for each $i$ we have
that $\edit_i \models \{\ParamVal_{i}\}\absEdit_i\{\ParamVal_{i+1}\}$.
%
Further, we write $\edit \models \absEdit$ and $\edit_0\ldots\edit_n \models
\absEdit_0\ldots\absEdit_n$ if there exist some $\ParamVal$ and $\ParamVal'$
that make the above relationships hold.


\begin{example}
  While the above definition is involved, the notion of in and out parameters
  is easy to explain with an example.
  %
  For the delete parameter followed by delete corresponding arguments from
  call-sites workflow, we want to constrain the method name and parameter
  name be shared across the two abstract predicates.
  %
  This is simply expressed as the sequence
  $\mathsf{DelParam}[\outparam{method}, \outparam{paramName}] \cdot
  \mathsf{DelArg}[\inparam{method}, \inparam{paramName}]$.

  Consider the following code fragment in Figure~\ref{fig:code}.
  %
  Let
    $\ParamVal_0 = \{\}$ and 
    $\ParamVal_1 = \ParamVal_2 = \{ \mathsf{method} \mapsto \code{Write},
    \mathsf{paramName} \mapsto \code{flush} \}$.
  %
  Abbreviating $\mathsf{method}$ as $\mathsf{m}$ and $\mathsf{paramName}$ as
  $\mathsf{pN}$, we have that:
  \begin{gather*}
    \edit_1
    \models
    \{\ParamVal_0\}\mathsf{DelParam}[\outparam{m},\outparam{pN}]\{\ParamVal_1\}
    \quad
    \edit_2
    \models
    \{\ParamVal_1\}\mathsf{DelArg}[\outparam{m},\outparam{pN}]\{\ParamVal_2\}
    \\
    \edit_1 \edit_2
    \models
    \{ \ParamVal_0 \} \mathsf{DelParam}[\outparam{m}, \outparam{pN}] \cdot \mathsf{DelArg}[\inparam{m}, \inparam{pN}] \{ \ParamVal_2 \}
  \end{gather*}

  On the other hand, there is no value of $\ParamVal$ and $\ParamVal'$
  which enforces $\edit_1\edit_4 \models
  \{\ParamVal\}\mathsf{DelParam}[\outparam{m}, \outparam{pN}] \cdot
  \mathsf{DelArg}[\inparam{m}, \inparam{pN}] \{ \ParamVal' \}$.
  %
  The abstract edit sequence along with the in and out parameter constraint
  exactly enforce that a delete parameter and a delete argument edits
  correspond to each other.
  \qed
\end{example}

\noindent\emph{Comparison to existing work.}
In the literature, the most common way of expressing parameter flow like
constraints is using ....
%
For example, $\mathsf{DelParam}[\outparam{m}, \outparam{pN}] \cdot
\mathsf{DelArg}[\inparam{m}, \inparam{pN}]$ is usually expressed as
...\cite{xxx}.
%
While this notion is significantly simpler, as we will see in the following
paragraphs, the parameter flow notion allows us to precisely express
extremely detailed and sophisticated edit patterns.



\begin{figure}
\small{
  \begin{alltt}
\minus{void Process(obj data, CancellationToken cancel) \{}
\plus{void Write(Stream s, byte[] bs) \{ // Edit 1}
  ...
\minus{ProcessHelper(cancel);}
\plus{ProcessHelper(); // Edit 3}
  ...
\minus{Persist(results, cancel);}
\plus{Persist(results); // Edit 5}
\}

\minus{void ProcessHelper(CancellationToken cancel) ...}
\plus{void ProcessHelper() ... // Edit 2}

\minus{void Persist(obj results, CancellationToken cancel) ...}
\plus{void Persist(obj results) ... // Edit 4}

void Main(string[] args) \{
\minus{  Process(args[0], new CTSource().Token);}
\plus{  Process(args[0]).Token); // Edit 6}
\}
  \end{alltt}
}
  \vspace{-3ex}
  \label{fig:code-cancel}
  \caption{Delete parameter from API}
\end{figure}

\begin{example}[Delete common parameter from API.]
  A very common task is to remove a common parameter from all the methods of
  an API.
  %
  For example, consider the code in Figure~\ref{fig:code-cancel}.
  %
  Here, all methods in the API accept a cancellation token argument which can
  be used to cancel the operations.
  %
  Now, the developer makes the full API non-cancellable by removing all the
  cancel parameters and arguments.
  %
  This edit pattern can be captured by the  pattern $\SeqPat = 
    \left(
      \mathsf{DelParam}(\outparam{m}, \outparam{pN}) \cdot
      \mathsf{DelArg}(\inparam{m}, \inparam{pN})^*
    \right)^\shuffleStar
  $.
  %
  This pattern restricts the delete argument edits for each method occur
  after the corresponding delete parameter edit, but the edits for different
  methods may be interleaved.
  \qed
\end{example}

\begin{figure}
\small{
  \begin{alltt}
\plus{Context GetContext() \{ ... \} // Edit 1}

\minus{void Entry(Context context)}
\plus{void Entry() // Edit 2}
\minus{\{  MidLevel1(context); \}}
\plus{\{  MidLevel1(); // Edit 3 \}}

\minus{void MidLevel1(Context context)}
\plus {void MidLevel1() // Edit 4}
\minus{\{  User(context); \}}
\plus{\{  User();  // Edit 5 \}}

\minus{void User(Context context)}
\plus{void User() // Edit 6}
\minus{\{  var y = context.GetProperty(x); \}}
\plus{\{  var y = GetContext().GetProperty(x); // Edit 7 \}}
  \end{alltt}
}
  \vspace{-3ex}
  \label{fig:code-cancel}
  \caption{Delete parameter from call chain}
\end{figure}

\begin{example}[Delete parameters from call chain]
  In a deeply nested call chain, often a single parameter is used at the
  bottom of the call chain is passed through every method above the call (see
  Figure~\ref{fig:code-call-chain}).
  %
  This style is sometimes considered an anti-pattern and developers often
  refactor code to avoid this style.
  %
  A common workflow to achieve this:
  \begin{inparaenum}[(a)] 
    \item Delete parameter from entry point (here \code{Entry});
    \item Find the next error (where the parameter is used in the current
      method) and delete the argument there (here call to \code{MidLevel1}); 
    \item Using the IDE's go to definition of the called function and delete
      the parameter in that location (here definition of \code{MidLevel1});
    \item Repeat until the bottom of the call chain is reached.
  \end{inparaenum}
  
  The sequence of edits can be represented using the edit sequence pattern $\SeqPat = 
     \mathsf{DelParam}(\outparam{m}, \outparam{pN}) \cdot
     \left(
       \mathsf{DelArg}(\outparam{m}, \inparam{pN}, \mathsf{location} \in \mathsf{Body}(\inparam{m})) \cdot
       \mathsf{DelParam}(\outparam{m}, \inparam{m}, \inparam{pN})
     \right)^*
  $.
  %
  This pattern precisely captures the described workflow, showing that the
  edit sequence pattern concept is highly expressive.
  \qed
\end{example}

\noindent\textbf{Applications.}
\arsays{Talk about the prediction thing?}



==> implications.tex <==

\section{Implications}
We discuss some main insights and learnings we gained from analyzing code edit data
using \technique.

\smallskip\noindent{\textbf{Existing automation tools are not used at their full potential.}}
\\
{\em{Observation:}} Modern IDEs provide support for automating several common code edits, refactorings,
or code fixes, but we still observe developers doing those changes by hand. 
\\
{\em{Analysis:}} We believe the reason is that this automation is hard to discover 
(discoverability issue), and even when it is discoverable, developer do not realize 
the possibility of using it at the time when that suggestion is available (late-awareness). 
\\
{\em{Action:}} The edit sequence patterns for tasks that are currently automated in IDEs
can be monitored and we can build telemetry to check how often people are not using available
tools.

\smallskip\noindent{\textbf{Improving current automation.}}
\\
{\em{Observation:}} We found new edit sequence patterns, along with some well-known patterns that are
currently automated.
\\
{\em{Analysis:}} There are a few automation tools ([BeneFactor, WitchDoctor, IntelliCode suggestions] 
that exploit temporal context. They observe the past edit(s) made by the developer to surface
the next edit suggestion. This way they are able to address discoverability and late-awareness 
issues. 
\\
{\em{Action:}} The new spatiotemporal edit sequence patterns we found can be used in the same way to
make edit suggestions.  The suggested edits can just be those that IDEs already implement, such
as quick actions in Visual Studio. They suggested edits can also be new quick actions. The main
benefit would be improved discoverability and eliminating late-awareness issues.
    

\smallskip\noindent{\textbf{Novel ways to exploit spatiotemporal context.}}
\\
{\em{Observation:}} Analysis of the edit sequences performed by developers revealed some patterns that do not directly fall into any class of existing automated code fixes or refactorings.
\\
{\em{Analysis:}} The new patterns suggest new ways to use the spatiotemporal context to suggestion edits.  
\\
{\em{Action:}} First, it may be possible to suggest a {\em{composition of quick actions}}; for example, 
if a developer has added 4 parameters to a constructor, we can make {\em{one}} suggested edit that
handles all 4 parameters simultaneously (as opposed to having the developer invoke some quick action 
4 times). The main benefit would be that we get automation of larger workflows without needing to implement a larger quick action.
\\
{\em{Action:}} Second, temporal context could be used to rank or filter out quick actions.
For example, when a developer changes the type of a returned expression, then
instead of showing the action to fix the expression, we show the action to fix the return type 
of the method.
As another example, when a develper creates a variable, we can filter out the
complaint that the variable is unused because in all likelihood the developer would
next use the variable. The main benefit here is that we are able to reduce noise 
in the UI.
\\
{\em{Action:}} Finally, copy-paste is a common pattern used for authoring code,
and temporal context can yield a smart copy and paste experience.
For example, after a developer does a copy-and-paste on a property, they next update 
the type and name in the pasted code.  
After a developer does a copy-and-paste on an if-condition, they update the variables next.
The temporal context can thus be used to help the developer modify the pasted code.
The main benefit is that we can help developers author code when copying and pasting. 

\smallskip\noindent{\textbf{Data-driven handling of feature requests.}}
\\
{\em{Observation:}} Several open feature requests for automation in IDEs can be mapped to
spatiotemporal edit sequence patterns we extracted using \technique.
\\
{\em{Analysis:}} The edit sequence patterns generalize the example provided in the feature request
and also provide details on their frequency.
\\
{\em{Action:}} Use information from the edit sequence patterns to prioritize feature requests,
and then use the temporal context to suggest the generalized edits in the pattern.


\ignore{
\section{OLD IMPLICATIONS}


\begin{enumerate}[wide, label=\bfseries I\arabic*., leftmargin=*, labelwidth=!, labelindent=0pt]

\item \textbf{Discoverability and Late-awareness}\gustavo{can you come up with a title/sentence to describe the implication? It will help you to write it. This title is not an implication but a problem.}: Our results (\Cref{tasksAndWorkflows}) reveal that developers perform programming tasks (like rename or change method signature) by hand rather than using the available automation\gustavo{I don't think we can say this for sure. We found manually applied things, but it does not mean that they did not use the tool other times.}. 
Currently IDEs offer over a 100 C\# refactoring, code-fixes or templates through quick actions and contextual menu to the user; and the IDE designers are striving towards more automation.
However, often developers are unable to \textit{discover} the available automation or they realize a particular automation was applicable when they are half way through performing the task manually. 
To solve this problem, the new generation of tools track the edits that developers perform to infer the user's intention and provide a appropriate suggestion to complete the task for the user. 
To develop such tools, IDE designers manually identify the common \textit{edit workflows} to perform the task, via user studies, video recordings and personal experience.
This approach is not scalable, specially given that there are many such automation that warrant tracking recent edits. 
\gustavo{until this part, it was kind of repetitive. It sounded more like the problem motivation that we wrote in the intro than an implication.}
In our study we show that \technique is effective and useful at unblocking this bottleneck.
Our thorough qualitative and quantitative analysis shows that \technique is effective at simplifying the identification of high-level programming tasks and their corresponding edit workflows and useful at finding specific edit sequence patterns.
Moreover, the catalog of programming tasks and edit workflows we created can be used a starting point to build this new generation of tools.

\item \textbf{Suggestions based on recent edits}: 
\gustavo{I think this paragraph is interesting but it is talking about too many things at once. We may want to separate each one of the aspects.}
We observed that developers apply common and predictable sequences of edits (\textit{edit workflow}) to perform a high-level programming task.
\gustavo{That's the big observation of your study. You may want to put this in the beginning of section 8, and then describe what are the implications of that observation.}

Modern IDEs provide automation for a large variety of these steps as code-fixes. 
However, this requires IDE designers to identify \textit{where} and \textit{when} to surface the suggestions for \textit{code-fixes}.
Currently IDE designers have to rely upon their personal experience and feedback from the user community to make such decisions.
\gustavo{this is a little bit confusing because you're introducing a new motivating problem at the end of the paper... it's like: wait... what? you only told me about this now?}

\technique alleviates this problem by reporting common edit sequences patterns performed by developers in practice. 
These patterns allow the IDE designers to explore the various scenarios where a developer would potentially invoke the automation. 
\gustavo{what are the implications for the problems that we mentioned in the intro?}

For instance, in \Cref{featureRequestResults} \technique found two new scenarios where surfacing the code-fix to \textit{fix return type} would be beneficial. 
\gustavo{I don't understand this example}

Moreover, IDE designer also have to decide the order in which the code-fix and refactoring suggestions appear in the contextual menu.
\gustavo{a new problem... I think these problems need to be better introduced.}

Our results highlight that developers\gustavo{we should try to avoid often since we are not presenting statistics} often perform an edit based on a recent edit.

However, currently the suggestions are ordered based on a pre-determined priority and its applicability to the current context\footnote{\url{https://github.com/dotnet/roslyn/issues/35525\#issuecomment-517028450}}; missing the crucial temporal aspect. 
The edit sequence patterns reported by \technique can be used to improve the suggestions provided in the contextual menu; enhancing the productivity of the developer.
\gustavo{I think this implication should have its own subsection}

\item \textbf{New opportunities for automation:}


\item \textbf{Making Data-Driven decisions}: 
While Visual Studio and Resharper provides over a 100 automations, there are still 10s of new code-fixes and refactorings that the users desire. 
The IDE designers not only have to filter feature requests that warrant a new feature, but also have to  prioritize the development of these features. 
Tool builders currently rely on their personal experience and user feedback to make these decisions. 
Now \technique empowers the IDE-designers to make data driven decisions by considering the real-world instances of a specific edit sequence pattern(s) where the proposed automation can be beneficial. 
IDE-designers can use this information prioritize the features based on their likelihood to be used in practice. 
\gustavo{you may want to add some concrete examples that our study found}

\item \textbf{Discovering under use of automation}: Currently, IDE-designers have deployed huge infrastructures\footnote{\url{https://docs.microsoft.com/en-us/visualstudio/ide/visual-studio-experience-improvement-program?view=vs-2019}} that  collects information about errors, computer hardware, and how people use Visual Studio, without interrupting users in their tasks at the computer. 
However, there are no means to gain insight into the under use of the offered automation (i.e. how many times developers manually performed the task instead of invoking the automation).
We show that \technique can effectively mine the edit workflow manually applied by the developer to perform a high-level programming task.
IDE-designers can add mechanisms to detect specific edit workflows that \technique identified to gain insight into the under use of specific high-level programming tasks, for which automation is offered. 
\gustavo{this is good}

\item \textbf{Coding not L -> R} ?

\end{enumerate}
}

==> introduction_fse2021.tex <==
\begin{itemize}
    \item \todo{motivating example} How to rewrite the motivating examples? It seems we have other aspects to emphasize.
    \item \todo{$\dependency$}
    \item \todo{Change figure to split summarize step into quotient and mine}
    \item \todo{Make the title case/sentence case in all paragraph headings uniform.}
    \item \todo{In RQ1, we should also compute threshold by sketch.}
\end{itemize}
\section{Introduction}

Integrated Development Environments (IDEs) offer developers an overwhelming deluge of tools to support source code editing tasks, including writing new code, performing refactorings, and applying code fixes. Popular IDEs such as Microsoft Visual Studio~\cite{visualstudio} and JetBrains ReSharper~\cite{resharper}, for example, provide over 100 C\# refactorings, code fixes, and snippet tools.

Unsurprisingly, developers have difficulty discovering these tools and applying them at the appropriate time and place~\cite{6112738}.
Toolsmiths have implemented tool recommenders in IDEs to support these developer challenges. For instance, if the developer clicks on a variable declaration, Visual Studio will suggest a quick action to invoke the Rename Variable refactoring tool. Such recommendations reason through a \emph{spatial context}, that is, the current location where the developer is editing the code.

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{figures/bluepencil.png}
\vspace{-4ex}
\caption{IntelliCode suggestions provides a temporal recommendation based on recent edits by the developer.}
\label{fig:bluepencil}
\vspace{-2ex}
\end{figure}

\begin{figure}[!t]
\centering
% \includegraphics[scale=0.8]{figures/rename-with-editor-cs.png}
\includegraphics[trim=0 0 200 0, clip, width=\linewidth]{figures/rename-2.png}
\vspace{-4ex}
\caption{Visual Studio temporally detects the name update from \code{Person} to \code{Employee} and suggests \textit{rename refactoring}.}
\vspace{-4ex}
\label{fig:manual-rename}
\end{figure}

%Although useful, a significant limitation of spatial recommendations that the same spatial context may be valid to many tools. Therefore, theis many tools can be that their solution space is often too large to be able to offer a useful recommendation
\ignore{Although useful, a significant limitation of spatial recommendations is that their solution space is often too large to be able to offer a useful recommendation, and there are certain recommendations that simply can't be expressed through a purely spatial context~\cite{7816468,Miltner:BluePencil}.}
%
While they are very useful, spatial context based tools do not
have the temporal context to precisely determine when they are applicable.
%
Hence, at any point, a significant fraction of these tools produce
suggestions that often obscure the desired one.
%
Further, there are entire classes of recommendations that cannot be
expressed in a purely spatial context~\cite{7816468,Miltner:BluePencil}.
Consequently, IDEs are now beginning to use previous edits performed by the developer in the IDE---that is, a \emph{temporal context}---to enable more expressive recommendations. For instance, Visual Studio recently released the Intellicode suggestions feature~\cite{Miltner:BluePencil,intellicode}. 
It tracks recent edits performed by a developer, identifies patterns of repeated edits, and generates suggestions to automate the remaining edits. 
Figure~\ref{fig:bluepencil} shows a suggestion produced by IntelliCode after the developer had performed two similar edits elsewhere in the code. 
While IntelliCode suggestions use the temporal context to identify repeated edits, BeneFactor~\cite{Ge:ICSE:RefactoringSteps} and WitchDoctor~\cite{witchdoctor} use the temporal context to detect that the developer is manually performing a refactoring and offer an edit suggestion to automate the remaining steps of the refactoring.
Visual Studio implements this idea to detect when a developer is manually renaming a variable and suggests an edit to finish the refactoring, as shown in Figure~\ref{fig:manual-rename}. 

The aforementioned examples demonstrate a desire for building tools that use spatial and temporal contexts. Through formative interviews with recommendation system toolsmiths of a popular IDE (two program managers and a principal software engineer), we found, however, that building tools that exploit both signals is challenging.  First, our toolsmiths reported that recognizing these signals is largely a manual process, without any data-driven approaches to recognize temporal patterns and how they interact with spatial signals. Second, developers use multiple, diverse strategies to make the same change, which makes it difficult for our toolsmiths to systematically understand and catalog what edits developers perform in practice. Third, our toolsmiths indicated that it is difficult for them to discover potentially valuable recommendations that do not currently exist, relying instead on manual bug reports or feature requests. Their reported challenges are similar to those of IntelliCode suggestions, BeneFactor and WitchDoctor~\cite{Miltner:BluePencil,intellicode,6112738,Ge:ICSE:RefactoringSteps}.

To address these challenges, we propose \technique, a technique for mining temporal patterns in sequences of edits applied in an IDE. 
\technique represents the fine-grained sequences of code edits applied in an IDE as a graph that captures temporal and spatial relationships among the edits. 
It then lifts this temporal and spatial information to a more abstract representation and reports the common patterns, for the toolsmiths to explore.

We conducted an empirical study to evaluate the usefulness of \technique\ from the
perspective of a toolsmith.
%
We instantiated \technique on a C\# corpus containing \numberOfHours hours of
development across \numberOfProjects code bases by \numberOfDevelopers developers
in a large software company.
%
%We identified \totalWorkflows temporal edit patterns related to \totalTasks distinct
%code editing tasks.
We identified \totalTasks temporal edit patterns related to existing features in Visual Studio 2019 or feature requests.
%
Our study suggests that existing automation is underused, and that, temporal edit patterns can offer toolsmiths support to build tools that combine temporal and spatial contexts to provide the right recommendation in the right location at the right time.
%Among these patterns, we found patterns corresponding to
%\technique detected patterns corresponding to 
%developers manually performing
%a sequence of editing actions that could have been automated using an existing tool.
%
%These patterns can be used to detect missed opportunities for using the tools
%\emph{during the manual sequence of actions}, paving the way for suggestions that
%automate the rest of the partially completed edit.
%
%Further, we also discovered new temporal edit patterns that are opportunities
%for building new automation tools.


The paper makes the following contributions: 
\begin{enumerate}
    \item We formalize the problem of mining temporal edit patterns;
    \item  We propose \technique, a technique for mining temporal patterns from fine-grained edits performed in an IDE;
    \item We demonstrated the usefulness of \technique by conducting an empirical study that results in a catalog of \totalTasks \textit{relevant} temporal patterns.  
    \item We present a \textit{actionable} set of implications of our findings from the perspective of \textit{toolsmiths} to better support their tools.
\end{enumerate}


==> introduction_prebarik.tex <==
\section{Introduction}

Integrated Development Environments (IDEs) provide tool support for several source code editing tasks, from writing new code to performing refactorings and code fixes. 
For instance, Microsoft Visual Studio~\cite{visualstudio} and JetBrains ReSharper~\cite{resharper} offer over 100 C\# refactorings, code fixes, and snippets. 
To recommend the most useful code edit, the IDE leverage the \emph{spatial context}, that is, the current location where the developer is editing the code. 
For instance, if the developer clicks on a variable declaration, Visual Studio will suggest a quick action to invoke the Rename Variable refactoring. 

Besides the spatial context, IDEs are starting to use the \emph{temporal context} to recommend code edits. By temporal context, we mean the previous edits performed by the developer in the IDE. 
For instance, Visual Studio recently released the Intellicode suggestions feature~\cite{Miltner:BluePencil,intellicode}. 
It tracks recent edits performed by a developer, identifies patterns of repeated edits, and generates suggestions to automate the remaining edits. 
Figure~\ref{fig:bluepencil} shows a suggestion produced by IntelliCode after the developer had performed two similar edits elsewhere in the code. 
While IntelliCode suggestions use the temporal context to identify repeated edits, BeneFactor~\cite{Ge:ICSE:RefactoringSteps} and WitchDoctor~\cite{witchdoctor} use the temporal context to detect that the developer is manually performing a refactoring and offer an edit suggestion to automate the remaining steps of the refactoring.
Visual Studio implements this idea to detect when a developer is manually renaming a variable and suggest an edit to finish the refactoring, as shown in Figure~\ref{fig:manual-rename}. 



%While tool support can automate time-consuming and error-prone programming tasks, they are often underused.  To effectively use the tool, a developer must be aware of the tools existence, and must know how to invoke it. A lack of this knowledge leads to the so-called \textit{discoverability} problem.
%Even if the tool is discoverable by the developer, the developer may not realize that they could
%invoke the tool at the start of a task. Instead, they could start doing the task manually, and only
%later realize that they could have invoked a tool to do the task. At this point, most of the
%developers finish the task manually~\cite{Ge:ICSE:RefactoringSteps}.  This late realization is
%referred to as the \textit{late awareness} problem.
%
%due to two common problems: \textit{discoverability} and \textit{late awareness}~\cite{Ge:ICSE:RefactoringSteps}. 
%Discoverability is related to the assumption that developers know that the tool exists and how to invoke it.
%Late-awareness is related to fact that developers often do not realize they could invoke a tool at the start of a task and thus they start the task manually and, only later, they realize they could have invoked a tool.
%At this point, most of the developers finish the task manually~\cite{Ge:ICSE:RefactoringSteps}. 

%\titus{The problem I see with this framing is that we don't actually ever show that we address discoverability and late awareness other than theoretically.}
%To address the discoverability and late awareness problems, researchers have proposed refactoring tools that detect when the developer is manually performing a refactoring and generate a suggestion to automate the remaining task~\cite{Ge:ICSE:RefactoringSteps,witchdoctor}.
%This idea can also be found in existing IDEs.
%For instance, when a developer manually updates the class name in Visual Studio, it suggests the \textit{rename refactoring}, as shown in Figure~\ref{fig:manual-rename}. 


\begin{figure}[!t]
\centering
\includegraphics[scale=0.5]{figures/bluepencil.png}
\caption{IntelliCode suggestions recommends a code edit based on a recent edit performed by the developer.}
\label{fig:bluepencil}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[scale=0.8]{figures/rename-with-editor-cs.png}
\caption{Visual Studio detects that the name was updated from \code{MyClass} to \code{Person} and suggests \textit{rename refactoring}.}

\label{fig:manual-rename}
\end{figure}

The success of aforementioned examples validate the approach of generating code edit suggestions using a combination of spatial and temporal context. However, building tools that exploit both signals is challenging. This is due to a lack of general knowledge on {\emph{temporal patterns}}, and how they interact with spatial signals, in edits performed by developers. The specific examples mentioned above relied on some very specific such knowledge. For example, IntelliCode suggestions focused only on repeated edits in a sequence. Meanwhile, to implement BeneFactor and WitchDoctor, tool builders have to identify the temporal patterns that represent developers manually applying a refactoring, which itself may require analyzing the video recordings of refactoring sessions~\cite{6112738,Ge:ICSE:RefactoringSteps}.
This approach does not scale to the vast number of tools -- beyond just repeated edits and specific refactorings -- that warrant this spatio-temporal context-sensitive automation.

% has the potential to solve the discoverability and the late-awareness problems. 
% However, before implementing them, tool builders have to perform two tasks. 
% First, they have to identify which tools suffer from these problems. Then, they have to identify the sequence edit patterns that corresponds to manually performing the tasks automated by these tools. So far, researchers have performed these tasks for a small set of refactorings by analyzing video recordings of refactoring sessions~\cite{6112738,Ge:ICSE:RefactoringSteps}. 
% Unfortunately, such an activity is time-consuming and does not scale.

\titus{I wonder if most of this can be moved to related work and perhaps some of the idea here can just be merged with the next paragraph. ``One possible way`` is a ``law of the instrument'' type of argument.}
One possible way to increase the knowledge in academia and industry about edit sequences is to use data mining.
In that regard, several mining techniques have been proposed to find edit patterns in source code repositories~\cite{getafix,revisar,refazer, Negara:ICSE:MiningEdits, Nguyen:CPatMiner}. 
Given two versions of the code in the repository, they can identify similar edits and generalize them into an edit pattern. Note, however, that these patterns do not explain {\ashish{the rich temporal flow that was used to perform the bigger changes that were committed to the repository.}} how developers performed the change that was committed to the repository. 
To obtain this information, there is a need for a technique that can mine {\ashish{spatio-temporal}} temporal patterns from the sequence of edits performed in an IDE.
%In that regard, several mining techniques have been proposed to find edit patterns (defined by single edits) in source code repositories~\cite{getafix,revisar,refazer, Negara:ICSE:MiningEdits, Nguyen:CPatMiner}, but there is a lack of techniques to mine patterns of {\em{edit sequences}} performed in an IDE.


\mohammad{This seems to be the key distinction of this paper and feels like the place that needs to be explained/motivated best in the intro. When reading the title, the first question that came to mind was how is this different from so much existing work on mining code patterns? It would be good to explain: (1) what is precise distinction between sequence of edit pattern vs edit patterns - why the latter cannot just include the former. (2) In terms of techniques, what is technically challenging or different about mining sequences of edit patterns vs. mining edit patterns. 
}
\gustavo{We updated the text but most of the challenges are shown in 2 but we can try to give an overview here.}

In this paper, we propose \technique, a technique for mining temporal patterns in the sequences of edits that developers perform in an IDE. 
The input for the technique is a dataset containing fine-grained sequences of code edits applied in any IDE. 
\technique\ can process such a dataset and create a graph representation of the edit patterns and their temporal and spatial relationships, which it stores internally.
\titus{I liked the story up until now. Is there anything we can see here stronger than ``can now be queried''; otherwise this is mostly a feasibility claim.}
The mined temporal patterns can now be queried by specifying parameters for the search. For instance, we can search for patterns applied by some minimum number of developers, or we can filter patterns based on how often it was applied. 
It is also possible to query by example, where the \technique reports all patterns that contain the provided example of edit(s).% that the pattern should subsume\ameya{contains?}. \technique returns all temporal patterns that meet the given specification. 

%The key technology behind \technique is an algorithm that generalizes the fine-grained edit sequences into a graph representation of the edit sequence patterns and  their temporal and spatial relationships. The temporal relationship allows the system to find sequences of edit patterns, and the spatial relationship allows it to identify how these sequences compose larger edits.

%Internally, \technique tree steps to a graph representation of the edit sequence patterns. 
%First, 
%Next, the  An edit sequence pattern generalizes similar sequences of edits applied multiple times, possibly by different developers. For instance, Figure~\ref{challenge:generalization} shows two similar edit sequences to add a property to a class and initialize it in the constructor. Note that the properties added in each sequence have different names and types but the structure of the edit sequences are the same. 
%\begin{itemize}
%    \item challenge one: generalizing edits
%    \item challenge two: granularity of the edits
%    \item challenge three: grouping edit sequence patterns together
%    \item challenge four: navigating the data
%\end{itemize}

We instantiated \technique on a C\# corpus containing \numberOfHours hours of code development performed by \numberOfDevelopers developers in a large software company. The developers were working on \numberOfProjects different code bases. 
We then performed two complementary studies to evaluate different ways that \technique can help researchers and tool builders find relevant temporal patterns. In the first study, we analyzed the most frequent temporal patterns returned by \technique. In the second one, we show how \technique can be used in a more guided way to search for specific patterns. To do so, we analyzed feature requests submitted to Visual Studio and Resharper and extracted examples of quick actions developers want to support for. We use these examples as inputs to \technique to find their corresponding temporal patterns.

In our studies, we identified \textcolor{red}{\totalWorkflows} temporal patterns related to \textcolor{red}{\totalTasks} distinct code editing tasks.  
Most of these temporal patterns were not reported in the literature or implemented by existing tools. 
They not only include temporal patterns related to a single quick action, but also patterns that represent the application of multiple quick actions. Additionally, our patterns show that developers use different edit sequences to perform not only refactorings, as already shown in previous studies, but also tasks related to creating and deleting code.
For instance, a common pattern for creating new code was to copy and paste a similar code and adapt it to the current context.
In section~\ref{s:discussion}, we discuss
how these patterns can be used by existing temporal-based tools and ideas for the development of new tools. 

%\begin{enumerate}
%    \item \textbf{Qualitative analysis} - 
%    The goal of our qualitative analysis is to increase the knowledge in the research and the industry communities on how developers code. To do so, we create a catalog of programming tasks and their corresponding edit sequence patterns. First, we searched on \technique for popular edit sequence patterns based on their occurrences and the number of developers that applied them. 
%Next, two authors of the paper collaborated on coding the 364 popular patterns using negotiated agreement techniques to achieve agreement. This analysis led to the identification of \textcolor{red}{25} programming tasks and \textcolor{red}{50} corresponding edit sequence patterns. %Moreover, we identified and formalized preconditions related to the shared information between the edits in the sequence to increase the confidence that the edit sequence pattern is related to the corresponding task.  
    
    % interesting facts 
 %   Our catalog contains X new edit sequence patterns for existing refactorings, Y patterns for creating new code, Z patterns related to applying refactorings in batch or in chain, besides patterns for deleting code and performing type changes. 
  %  Additionally, our study suggests that developers use different edit sequences to perform not only refactorings, as already shown in previous studies, but also tasks related to authoring and deleting code. For instance, while we have not found patterns for creating class properties using the snippet shown in Figure~\ref{fig:prop}, a common pattern found for this task is to copy and paste an existing property and change its name and type. 
    
  %   \item \textbf{Quantitative analysis} The goal of our quantitative analysis is to evaluate \technique's effectiveness in searching for edit sequence patterns using examples. We collected 21 feature requests submitted to Visual Studio and ReSharper related to edit automation. All these requests had examples of the edit the user wants to automate. \technique returned edit patterns for 12 of these feature questions with overall precision of 75.2\%. Our results suggests that \technique can be used to help tool builders to prioritize feature requests by analyzing how often the changes are performed in practice. 
%\end{enumerate}

The paper makes the following contributions: 
\begin{enumerate}
    \item We formalize the problem of mining temporal patterns;
    \item  We propose \technique, a technique for mining temporal patterns from fine-grained edits performed in an IDE;
    \item We demonstrated the usefulness of \technique by performing two complementary studies that resulted on a catalog of \textcolor{red}{\totalTasks} mined temporal patterns and their corresponding tasks.  
\end{enumerate}

%We applied \technique on a corpus containing 250 hours of code development performed by 12 developers working on 2 different code bases~\gustavo{I wonder if there is a better way to describe this. People were working on more than 2 projects}. We designed two studies to evaluate our technique’s effectiveness and usefulness,
% we answer the following research questions: 
 
 
 %\begin{enumerate}
  %   \item \textbf{(Usefulness)} – \textit{Can our technique be used to query for real world instances of a desired edit sequence}?  To show that the tool can be useful for tool builders to make data-driven decisions, we query for edit sequence patterns for which users desire automation. We systematically analyzed the feature requests of 2 tool builders (Visual Studio and Resharper), to create a dataset of 24 useful edit sequence patterns. Evaluating the technique on our corpus revealed that, 23 out of 24 patterns could be expressed and at least one instance was found for 17 out of the 24 patterns. Further, manual validation revealed the accuracy to be 70\%. 
   %  \item \textbf{(Effectiveness)}- \textit{Does our approach simplify the identification of meaningful high-level program transformations performed in the IDE?}  We performed thematic analysis upon 100 most frequently applied edit sequence patterns, to compile a catalog of 6 frequent high-level program transformations performed in the IDE. Our analysis reveals many new edit sequence patterns (that were previously unknown), insights into how developers evolve code in their IDEs and highlight new automation opportunities for tool builders. 
 %\end{enumerate}


%When developers perform their day-to-day code development activity, they apply sequences of edits that are repetitive or inter-dependent in nature, forming an edit sequence pattern. 
%For instance, in \Cref{fig:PropertyDomain} (Top) a new property named \code{Id} is added to the class \code{Node}, then a similarly named parameter \code{id} is added to its constructor and then the property \code{Id} is assigned to the parameter \code{id}.
%IDEs assist developers to apply such edit sequences by offering automation for certain step in the sequence, in the form of a refactoring or a Quick action. For example, VS provides a quick action at the property to add an appropriate parameter in the constructor. IDE designers are now trying to further boost developer productivity by automating edit sequences by offering advanced code fixes or editor intelligence. For example, VS provides a quick action at the property, to insert a parameter and the initializer in one action. Moreover, modern IDEs provide intelligent features that observes the edits that a user is applying, understands the user’s intent to perform a certain refactoring or a repetitive edit sequence and complete the task for the user.  

%Developers and tool builders highly desire more automation that boosts productivity.  However, tool developers must rely on feature requests and customer feedback to identify candidate edit sequence patterns for automation. This is because there are no techniques that allows tool builders to explore the edit sequence patterns performed in the real world. This also prevents tool builders from making data-driven decisions when developing new automations. 

%While the IDE designers are striving to advance the tooling to automate the application of edit sequences in an IDE, this has been a blind-spot for researchers. The techniques proposed by previous researchers to mine code change pattern, use coarse-grained VCS snapshots. It is impossible to perform analysis that involves a temporal aspect of the edits applied in an IDE using a VCS snapshot. Recent researchers that used more fine-grained data directly from the IDEs focused on finding most applied code change pattern (single large edit, not edit sequences). However, they miss the temporal aspect of how edits are applied in a sequence. Previously, researchers also developed techniques to understand how developers applied edit sequences in an IDE but only in context of refactoring. 

%A technique to explore edit sequence patterns performed in the IDE by real-world developers, will give insight into how the code is evolved edit by edit. It will reveal new opportunities for tool developers to advance and improve the IDE intelligence for enhancing the user experience.  For instance, they can develop new code fixes that automate the most applied edit patterns, rank the suggested code fixes based on the recently applied edits or learn frequently applied edit sequence patterns on the fly. Further, if the tool builders can query for the real-world instances of a candidate edit sequence pattern, they will be able to make data-driven decisions when developing new automations. It will also empower researchers to understand how the code is developed before it is committed into the VCS…..

%The biggest challenge posed by our problem, is to mine continuous sequence of edit applied by the developer, without any knowledge of what the edit is and where a logical edit starts or ends. This makes it further challenging to infer the start and end of an edit sequence patterns.  …….

%In this paper, we propose a technique that can explore edit sequence patterns from fine-grained sequences of code changes applied in the IDE.  Our approach not only allows to rank the edit sequence patterns based on statistics (like frequency, number of developers who applied it or number of sessions in which it was applied) but also allows to query for real-world edit sequence pattern instances using examples of one or more edits. We applied our algorithm on a corpus containing 250 hours of code development performed by 12 developers working on 2 different code bases. We designed two studies to evaluate our technique’s effectiveness and usefulness,
% we answer the following research questions: 
% \begin{enumerate}
%     \item \textbf{(Usefulness)} – \textit{Can our technique be used to query for real world instances of a desired edit sequence}?  To show that the tool can be useful for tool builders to make data-driven decisions, we query for edit sequence patterns for which users desire automation. We systematically analyzed the feature requests of 2 tool builders (Visual Studio and Resharper), to create a dataset of 24 useful edit sequence patterns. Evaluating the technique on our corpus revealed that, 23 out of 24 patterns could be expressed and at least one instance was found for 17 out of the 24 patterns. Further, manual validation revealed the accuracy to be 70\%. 
%     \item \textbf{(Effectiveness)}- \textit{Does our approach simplify the identification of meaningful high-level program transformations performed in the IDE?}  We performed thematic analysis upon 100 most frequently applied edit sequence patterns, to compile a catalog of 6 frequent high-level program transformations performed in the IDE. Our analysis reveals many new edit sequence patterns (that were previously unknown), insights into how developers evolve code in their IDEs and highlight new automation opportunities for tool builders. 
% \end{enumerate}


%Our findings have actionable implications for many audiences. ….

==> motivating-example-draft.tex <==
\section{Motivating Example}
\label{sec:motivating-example}

\begin{figure}
  \scriptsize
%
% \centering
\hfill
%
\begin{subfigure}{0.30\textwidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize
]
  class Node {
  
    Node() {
    }
  }
\end{lstlisting}
\vspace{-6ex}
  \caption{$\version_0$}
\end{subfigure}
%
\hfill
%
\begin{subfigure}{0.30\textwidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
+   public str Id { }
    Node() {
    }
  }
\end{lstlisting}
\vspace{-6ex}
  \caption{$\version_1$}
\end{subfigure}
%
\hfill
%
%
% \hfill
%
\begin{subfigure}{0.30\textwidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
-   public str Id { }
+   public str Id {get;}
    Node() {
    }
  }
\end{lstlisting}
\vspace{-6ex}
  \caption{$\version_2$}
\end{subfigure}
%
\hfill

\hfill
%
\begin{subfigure}{0.30\textwidth}
  \begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
-   public str Id {get;}
+   public str Id {get;set;}
    Node() {
    }
  }
  \end{lstlisting}
\vspace{-6ex}
  \caption{$\version_3$}
\end{subfigure}
%
\hfill
%
%
%  \hfill
%
\begin{subfigure}{0.30\textwidth}
  \begin{lstlisting}[
  mathescape,
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
    public str Id {get;set;}
-   Node() {
+   Node(str id) {
 
    }
  }
  \end{lstlisting}
\vspace{-6ex}
  \caption{$\version_4$}
\end{subfigure}
%
\hfill
%
\begin{subfigure}{0.30\textwidth}
  \begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
    public str Id {get;set;}
    Node(str id) {
+     Id = id;
    }
  }
  \end{lstlisting}
%
\hfill
%
\vspace{-6ex}
  \caption{$\version_5$}
\end{subfigure}
\vspace{-2ex}
  \caption{Development Session: Syntactically correct versions
  while adding and initializing a property.}
  \label{fig:dev-session}
\vspace{-7ex}
\end{figure}

\begin{figure*}[t]

\begin{subfigure}{0.90\textwidth}
\centering
\begin{tikzpicture}[main/.style = {draw, circle}]
% \tikzstyle{box}=[
%       draw,
%       rectangle,
%       minimum width=2.00cm,
%       minimum height=0.75cm,
%     ]
\node[] (before) {
    \begin{lstlisting}[
          basicstyle=\ttfamily\scriptsize,
        ]
classDefinition{
    ...
    ...
}
    \end{lstlisting}};
    
\node[right of=before, xshift=4cm] (after) {
    \begin{lstlisting}[
        mathescape,
        language=diff,
        basicstyle=\ttfamily\scriptsize,
        ]
classDefinition{
    ...
+   public Hole_1 Hole_2 {get; set;}
    ...
}
    \end{lstlisting}};
\draw[->](before) -- (after); 
\end{tikzpicture}
\caption{$
      \mathsf{AddProperty}$}
\end{subfigure}

\begin{subfigure}{0.90\textwidth}
\centering
\begin{tikzpicture}[main/.style = {draw, circle}]
\node[] (before) {
    \begin{lstlisting}[
          basicstyle=\ttfamily\scriptsize,
        ]
ParameterList(
    ...
    ...
)
    \end{lstlisting}};
    
\node[right of=before, xshift=4cm] (after) {
    \begin{lstlisting}[
        mathescape,
        language=diff,
        basicstyle=\ttfamily\scriptsize,
        breaklines=false,
        ]
ParameterList(
    ...
+   Hole_1 Hole_2_LC,
    ...
)
    \end{lstlisting}};
\draw[->](before) -- (after); 
\end{tikzpicture}
\caption{$
      \mathsf{AddConstructorParameter}$}
\end{subfigure}

\begin{subfigure}{0.90\textwidth}
\centering
\begin{tikzpicture}[main/.style = {draw, circle}]
\node[] (before) {
    \begin{lstlisting}[
          basicstyle=\ttfamily\scriptsize,
        ]
MethodDefinition{
    ...
    ...
}
    \end{lstlisting}};
    
\node[right of=before, xshift=4cm] (after) {
    \begin{lstlisting}[
        mathescape,
        language=diff,
        basicstyle=\ttfamily\scriptsize,
        breaklines=false,
        ]
MethodDefinition{
    ...
+   Hole_2 = Hole_2_LC;
    ...
}
    \end{lstlisting}};
\draw[->](before) -- (after); 
\end{tikzpicture}
\caption{$
      \mathsf{AddAssignment}$}
\end{subfigure}
\caption{Example of an Edit Sequence Pattern learned by \technique for the workflow $
      \mathsf{AddProperty}
\cdot \mathsf{AddConstructorParameter}
\cdot \mathsf{AddAssignment}$. The variable component of the pattern are represented by \code{Hole}, with \code{Hole\_LC} being its lower case transformation. Note how the \code{Hole}s are shared among the different edit patterns. }
  \label{fig:devSession }
\end{figure*}

Figure~\ref{fig:dev-session} depicts a sequence of versions produced when a
developer is editing code in an IDE.
%
Here, the developer is creating and initializing a new property to a class.
%
In this sequence, the developer is making $3$ separate ``logical'' edits:
\begin{inparaenum}[(a)]
  \item adding a new property \code{Id},
  \item adding a new parameter \code{id} to the constructor, and
  \item adding a statement assigning the parameter to the property.
\end{inparaenum}
%
The sequence \emph{add property}, \emph{add constructor parameter}, and
\emph{assign property} is a temporal edit pattern that commonly recurs in
development sessions, across multiple developers.

\ignore{
Most IDEs offer tool support to automate each of above actions based on
the spatial context, i.e., where the cursor is placed currently.
%
For example, when the cursor is placed on the property declaration, Visual
Studio offers a quick action to automate the rest of the sequence.
%
On the other hand, it does not produce the suggestion when the developer adds
the property declaration and then navigates the cursor over to the
declaration of the constructor.
%
This severely reduces the value of these IDE features because of the \emph{late awareness}
problem~\cite{Ge:ICSE:RefactoringSteps,witchdoctor}: the developer does not realize that they are performing a
known sequence of actions.
%
As shown by ~\citet{Ge:ICSE:RefactoringSteps}, late awareness is one of the primary reasons for
underuse of IDE tools and automated refactorings.

\arjun{Mention different orders here? I think that is better in the implications?}

\gustavo{I think we should change this story. It does not reflect what we are currently implementing. Does it? Now, with gray text, we want the user to go to the location. This is also how we evaluate the tool} \priyanshu{Modified the story to take this into account}
An alternative solution is to combine spatial context with \emph{temporal
context}.
}

In the example discussed above, when the cursor is over the constructor declaration, the fact that the developer added a new property immediately prior is a strong hint that the
suggestion to add the parameter is relevant. Subsequently, when the user moves the cursor inside the body of the constructor, the previous two changes hint that the next change may be to initialize the property. Similar to this, there are many such sequential edits that are used frequently by developers to carry out routine tasks. However, only a handful of these patterns are available as recognized easy-to-use features in IDEs.

The (problem) being that the available suggestion techniques use either the spatial context or the temporal context, but do not combine both. Several instances of these patterns though frequently used are not obvious when referring to just one of the available contexts. \priyanshu{We need to reword it, is extremely hard to understand what's going on here ->} \yasharth{Reworded, example moved from later to here}For example, in Figure~\ref{fig:extract-constant},
the user introduces a new local variable \textit{Limit} that stores an \textit{Integer Constant} 1000. In the next steps, all usages of the constant in the current scope are replaced by the newly introduced variable. Here the temporal dependency between these consecutive set of edits is not evident if not for careful analysis of both the user's recent edit history and location of these edits.

%%% EXAMPLE 
\begin{figure}
  \footnotesize
  \hspace{2ex}
\begin{subfigure}[t]{0.3\linewidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize
]
// Edit 1
+int Limit = 1000;                         
 if (IsEmpty(b))
   return 1000;
 else if (IsEmpty(a))
   return 1000/b.Len;
 else
   return a.Len;
\end{lstlisting}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[t]{0.3\linewidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize
]
// Edit 2
 int Limit = 1000;                         
 if (IsEmpty(b))
-  return 1000;
+  return Limit;
 else if (IsEmpty(a))
   return 1000/b.Len;
 else
   return a.Len;
\end{lstlisting}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[t]{0.3\linewidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
// Edit 3
 int Limit = 1000;                         
 if (IsEmpty(b))
   return Limit;
 else if (IsEmpty(a))
-  return 1000/b.Len;
+  return Limit/b.Len;
 else
   return a.Len;
\end{lstlisting}
\end{subfigure}
\hspace{-6ex}
%
\vspace{-4ex}
  \caption{Manually applied introduce constant refactoring.}
  \label{fig:extract-constant}
\vspace{-4ex}
\end{figure}


\ignore{\arjun{Add a non-obvious example to hint at the difficulty in modeling these
temporal edit patterns}}
% Moreover, participants in user studies are prone to social-desirability biases which may lead to unnatural workflows. 

Designing suggestion tools based on temporal context requires insights
into the common temporal edit patterns in the sequence of edits performed by
developers.
%
User studies to collect these insights are not straight-forward to design and also expensive to conduct. Moreover, in these user studies, the user behaviour might not be the same as in an un-monitored environment. An alternative solution for extracting these insights can be to observe developers naturally interacting with an IDE session to edit code. We can use these log of edits across multiple IDE sessions to identify recurring temporal edit patterns for multiple developers in different contexts. But, how to extract these insights from a collection of series of file versions? Moreover, say we have these workflows, how to create predictive representations capturing different contextual variations? 


\ignore{Using such data can enable us to capture natural editing workflows and also potentially provide us automated feedback on the effectiveness of the suggestion tools.
However, manually analyzing such data is extremely hard as a developer may perform a very large number of edits in a relatively short duration of time ( a few thousand edits in as less as 2 hrs of development). Similarly converting the data to useful tools isn't stra  While there have been attempts to make systems for automated extraction of edits from data \cite{getafix}, to the best of our knowledge
}
\ignore{An automated tool that captures and suggests these temporal edit patterns would enable developers save a lot on time and resources spent over such common workflows.}
%
\yasharth{Research objective, cut down on the above para. Do we still nee to add this as our problem is now well desrcibed in the Intro?}
\ignore{

However, these insights are not easy to obtain through mining version control
data: the relevant fine-grained sequence of edits are lost when the developer pushes
the change as a single commit to the version control history.

\gustavo{Should we change this last part? We are not proposing to mine patterns to get insights anymore. Our patterns can be used to automate these changes.}

}

\ignore{
However, to our knowledge, no IDE provides an automated tool or snippet to
perform all three of these edits at once.
\gustavo{what do you mean by all three at once? I don't think this is what we
want right? the user would perform the first edit manually, and we can
predict the next 2? Btw, VS already supports this scenario but it is using
spatial information. If the user leaves the line where he added the property,
the suggestion goes away. I think we should use this example to show exactly
the benefit of adding the temporal aspect. Even if the user goes to the next
location (parameter list), we can offer the suggestion based on the temporal
aspect. We can also say that there are many ways to apply this pattern. For
instance, some users will start from the statement? }
%

\begin{itemize}
  \item Spatial context vs temporal context 
    -- spatial context doesn't show in add param location
    -- don't show for random properties (only for the one just added)
  \item Late awareness
  \item For temporal context, tool developer needs to understand the kind of
  sequences.
\end{itemize}

Adding a snippet or tool to perform all the actions in an edit sequence
pattern is not difficult in itself.
\gustavo{I don't think we should go there... I think we should talk about detecting a pattern instead of performing it.}
%
However, there are $2$ major issues facing an toolsmith in adding such tools:
\gustavo{I think it may be risky to follow this directions... I think we should focus on the temporal aspect only. There are other techniques to mine patterns in the repository that can be used to priorize feature requests.}
%
\begin{itemize}
  \item \emph{Which edit sequence patterns should be automated?}
    Currently, there is no systematic way of discovering new edit sequence
    patterns.
    %
    Either, an toolsmith has to check feature requests or has to manually
    analyze video recordings of development sessions~\cite{Ge:ICSE:RefactoringSteps}.
    %
  \item \emph{If automated, how often is will the tool be used?}
    Once an edit sequence pattern is found, the toolsmith has to make a
    decision as to whether it is worth spending time and resources on
    automating this pattern.
    %
    Again, there is no existing technique that will automatically determine
    how often such edit sequence patterns occur in real development sessions.
    %
  \item \emph{How should these sequences be automated?}
\end{itemize}
}

To this end, we develop \technique, a data-driven automated technique which aggregates common editing workflows like $
      \mathsf{AddProperty}
\cdot \mathsf{AddConstructorParameter}
\cdot \mathsf{AddAssignment}$ for multiple developers across IDE editing sessions to extract temporal edit patterns . These temporal edit patterns can then be used to provide contextualized suggestions to users based on their recent fine-grained edit history. 
Further, not every temporal edit pattern is a simple sequence of individual
edits.
%
For example, removing a parameter from a method declaration and then updating
all its call-sites by removing the corresponding argument is the sequence
$ 
      \mathsf{DeleteParameter}
\cdot \mathsf{DeleteArgument}^*
$, where the $(^*)$ stands for Kleene star.
%
In general, our temporal edit patterns are given by regular expressions over
individual edit patterns.
%
\arjun{Add an explicit overview of the edit patterns. Try to add an explicit edit pattern.}

Figure 5 describes an edit sequence pattern learned for the \emph{add property}, \emph{add parameter}, and \emph{assign property} temporal edit pattern. Each individual transition represents the \emph{before} and \emph{after} state of an edit sketch. We see that the \textit{type} and \textit{identifier name} in the \emph{add property} sketch in Fig 5(a) are represented by holes. This signifies that users make this edit at multiple different instances with some pieces of information specific to the context of the edit. Similarly, there are holes which cannot be concretely populated in the subsequent edit sketches in Fig 5(b) and 5(c). However, if we look carefully, these holes might be bound in time across sketches as the user carries out these sequential changes to add and initialize a property. In this case, the \textit{type} of the constructor parameter added is same as that of the property added, the parameter name is a \textit{lower case} version of the name of the property, and the property is being initialized to the parameter inside the constructor. Thus, what we end up with is multiple such editing workflows, the gaps in which could be filled using the current context in order to predict the next set of concrete changes in the workflow for the user.

We discuss three challenges in learning temporal edit patterns.

\noindent\textbf{Level of Granularity.}
In Figure~\ref{fig:dev-session}, the edit $\version_0 \to \version_3$ plays
the role of \emph{add property} in the ``add property, add parameter, and
initialize property'' sequence.
%
However, in the development session, this edit is not a single change, but a
sequence of changes $\version_0 \to \version_1$, $\version_1 \to \version_2$,
and $\version_0 \to \version_3$.
%
To produce the above temporal edit pattern, \technique has to consider the
development session at the granularity of $\version_0 \to \version_3$ instead
of the $3$ individual fine-grained edits.

% \mohammad{what is the reason for this? is it because the edit pattern is more general if the details of the three steps are allowed to be different? If so may be good to explain rather than just state the need.}

However, $\version_0 \to \version_3$ might have to be
considered at a finer granularity in a different context.
%
If we were exploring how developers add new properties
(not what developers do before and after adding properties), each of
$\version_0 \to \version_1$, $\version_1 \to \version_2$ and
$\version_2 \to \version_3$ is relevant.
%
\ignore{
By examining the add property edit in more fine grained manner, we were able to
discover different patterns of performing the add property action: some
developers simply type the declaration left to right and others copy-paste an
existing property and change the type and the name.
\gustavo{Should we link this paragraph to the discussion in section 5.1. We talk about this example.}
\ignore{
For example, one common recurring edit pattern is to make all properties of a
single class settable (this pattern occurs, for example, when making a class
JSON deserializable).
%
In this setting, we need to consider $\version_2 \to \version_3$ its own
separate edit and not a part of a larger edit.
}
}
Hence, depending on the scenario we are examining, the edits
may need to be ``grouped'' or ``sub-divided'', i.e., the session needs to 
considered at different levels of granularity.
% and considering patterns among the logical edits does not work.
%
% To answer queries about different scenarios and workflows, we need to examine
% the sessions at multiple granularities.

\noindent\textbf{Level of Generalization.}
The scenario of interest not only changes the appropriate granularity of edits, but also the level of generality of a single edit. 
%
In the session, the edit $\version_0 \to \version_3$ could be
considered under different levels of generalization, e.g., ``insert an  AST node'' ,
``insert a property'', ``insert a get-set property'', etc.
%
While coming up with the "ideal"
predictive representations of the temporal edit pattern for add and initialize property scenario $\version_0 \to \version_3$ should be regarded as  the insertion of a property,
not just any AST node.
%
However,  that $\version_0 \to \version_3$ adds a get-set
property is irrelevant, only that it adds a property.
%
Therefore, apart from different levels of granularity, we also need to
consider each single edit at different levels of generalization. 

\ignore{
\st{Since, it is  not always clear which generalization is the \textit{best} one for a given edit workflow, we list temporal edit patterns representations at varying degrees of generalizations and use a data-driven approach to pick a subset of most useful representations.}
\gustavo{this paragraph is hard to understand. Wouldn't be better to mention the AHC here?} \priyanshu{Removing this line seems to restrict the scope of this challenge to specify the "need". We can either just remove the strike throughed line or add some description of AHC}
% \yh{I believe we did not distinguish ``insert a property'', ``insert a get-set property'' in the sketches of edit sequence pattern.}
}

\mohammad{Granularity seems to almost be a special case of generalization, as being more granular can still be a more specialized edit pattern sequence - can we distinguish the two any further? (I think its also ok to leave it as is if not). Also, it is not clear what the notion of "correctness" here is - since a group of specialized patterns may serve the same purpose as a single generalized pattern and make the same suggestions to the user - perhaps we can comment on how in practice it is problematic to infer many specialized patterns? Like they dont generalize well to unseen data or become hard to manage or something?}

\noindent\textbf{Capturing Temporal Dependencies} When a user goes on to make a sequence of edits, oftentimes the subsequent edits possess relationships with recent edits which are essential to be modelled for a useful predictive representations of temporal edit patterns. In Figure~\ref{fig:dev-session}, the \textit{type} attribute of the newly added parameter in the $\mathsf{AddParameter}$ must be the same as the type  of the property in the $\mathsf{AddProperty}$ in the first step. Similarly, the \textit{identifier} for the property is same as that in the $\mathsf{AddAssignment}$. Standard practices in development also warrant a \textit{lowercase} version of the property identifier being used as the parameter identifier as well as in the $\mathsf{AddAssignment}$ later. Recognizing and mapping these relationships between entities of these edits in time is non-trivial. An expressive language is needed to represent these temporal dependencies across edits.  

\ignore{
\noindent\textbf{Temporal Summarization.}
%
\ignore{
\mohammad{the terms "temporal" and "sequential" are being used interchangeably and may be better to consistently use one to avoid confusion. It seems it is less about "temporal" but more about sequence and order-sensitivity of edits.
@Mohammad: We have had quite a bit of trouble with this nomenclature of
sequential and temporal. If you have a suggestion, we can discuss it.
}
}
%
\gustavo{We may want to delete this paragraph. The current technique is not handling this problem.}
Different developers perform the same logical edit using completely
different steps.
%
In Figure~\ref{fig:add-property-pattern}\gustavo{Fix the reference?}, the developer performs the edits
in the sequence add property, add constructor parameter, and add assignment.
%
However, some developers use the order add constructor parameter,
add assignment, and then, add property.
%
A toolsmith is often interested not in any single sequence, but a summary
of all sequences used by developers to perform the logical edit.
%
Hence, apart from finding the edit sequence pattern at the right granularity
and generalization in one session, we need to do so across multiple sessions
and summarize all these sequence patterns into a single temporal edit pattern 
that represents all ways of performing the same logical edit.
% \priyanshu{We still create temporal edit patterns at different granularity right? I am afraid having this description may warrant a discussion later in the paper about how the templates we have generated are at the "right" granularity and generalization which is currently missing.}
}
%
%%% OLD STUFF %%%
\ignore{
\gustavo{I think it's better change the example here by the one
where the developer perform the same set of actions using a
different order. It will make it easier to understand.}
 \arsays{Don't know what to call this.}
\gustavo{How about using the same example. We can say that a change would be
to perform 2 add properties, then 2 parameters, then 2 assignments. The
pattern would be: AddProperty*AddParameter*AddAssignment*?}
}
%
\ignore{
In many scenarios, individual temporal edit patterns may be combined into a
single, more general, temporal edit pattern.
%
For example, for add and initialize property task, different developers order
the individual edits in different ways.
%
In fact, we found instances of developers completing this task in all $6$
permutations of the three sub-steps.
%
We combine all these $6$ permutations into one temporal edit pattern
$
\{\!|  
\mathsf{AddProperty},
\mathsf{AddConstructorParameter},\\
\mathsf{AddAssign}
|\!\}
$, where
$\UnorderedSeq{\cdot}$ represents an unordered collection of individual
edit patterns.
%

%
This task of summarizing individual edit sequences into a regular
expression-like temporal edit pattern is not straight-forward often needs
human guidance.
\gustavo{I think we need to improve this part, right? 
\arjun{Yes, I will change this looking at sec 5 and 6}
}
}

\ignore{
\mohammad{until now we do a good job of motivating the problem and challenges, but the intro gives no insight into the techniques used to address the challenges (just that we have created a system that does so, which may give the impression that we may be lacking in interestingness of approach).
\arjun{This is a style thing. SE papers often use this -- I haven't used it before either.}
}
}

==> motivating-example-fse2021.tex <==
\section{Motivating Example}
\label{sec:motivating-example}

\begin{figure}
  \scriptsize
%
\hfill
%
\begin{subfigure}{0.20\textwidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize
]
  class Node {
  
    Node() {
    }
  }
\end{lstlisting}
\vspace{-6ex}
  \caption{$\version_0$}
\end{subfigure}
%
\hfill
%
\begin{subfigure}{0.20\textwidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
+   public str Id { }
    Node() {
    }
  }
\end{lstlisting}
\vspace{-6ex}
  \caption{$\version_1$}
\end{subfigure}
%
\hfill
%

%
\hfill
%
\begin{subfigure}{0.20\textwidth}
\begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
-   public str Id { }
+   public str Id {get;}
    Node() {
    }
  }
\end{lstlisting}
\vspace{-6ex}
  \caption{$\version_2$}
\end{subfigure}
%
\hfill
%
\begin{subfigure}{0.20\textwidth}
  \begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
-   public str Id {get;}
+   public str Id {get;set;}
    Node() {
    }
  }
  \end{lstlisting}
\vspace{-6ex}
  \caption{$\version_3$}
\end{subfigure}
%
\hfill
%

%
\hfill
%
\begin{subfigure}{0.20\textwidth}
  \begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
    public str Id {get;set;}
-   Node() {
+   Node(str id) {
 
    }
  }
  \end{lstlisting}
\vspace{-6ex}
  \caption{$\version_4$}
\end{subfigure}
%
\hfill
%
\begin{subfigure}{0.20\textwidth}
  \begin{lstlisting}[
  language=diff,
  basicstyle=\ttfamily\scriptsize,
  breaklines=false
]
  class Node {
    public str Id {get;set;}
    Node(str id) {
+     Id = id;
    }
  }
  \end{lstlisting}
%
\hfill
%
\vspace{-6ex}
  \caption{$\version_5$}
\end{subfigure}
\vspace{-2ex}
  \caption{Development Session: Syntactically correct versions
  while adding and initializing a property.}
  \label{fig:dev-session}
\vspace{-7ex}
\end{figure}

Figure~\ref{fig:dev-session} depicts a sequence of versions produced when a
developer is editing code in an IDE.
%
Here, the developer is creating and initializing a new property to a class.
%
In this sequence, the developer is making $3$ separate ``logical'' edits:
\begin{inparaenum}[(a)]
  \item adding a new property \code{Id},
  \item adding a new parameter \code{id} to the constructor, and
  \item adding a statement assigning the parameter to the property.
\end{inparaenum}
%
The sequence \emph{add property}, \emph{add constructor parameter}, and
\emph{assign property} is a temporal edit pattern that commonly recurs in
development sessions, across multiple developers.

Most IDEs offer tool support to automate each of above actions based on
the spatial context, i.e., where the cursor is placed currently.
%
For example, when the cursor is placed on the property declaration, Visual
Studio offers a quick action to automate the rest of the sequence.
%
On the other hand, it does not produce the suggestion when the developer adds
the property declaration and then navigates the cursor over to the
declaration of the constructor.
%
This severely reduces the value of these IDE features because of the \emph{late awareness}
problem~\cite{Ge:ICSE:RefactoringSteps,witchdoctor}: the developer does not realize that they are performing a
known sequence of actions.
%
As shown by ~\citet{Ge:ICSE:RefactoringSteps}, late awareness is one of the primary reasons for
underuse of IDE tools and automated refactorings.
%
% \arsays{Mention different orders here? I think that is better in the implications?}

An alternative solution is to combine spatial context with \emph{temporal
context}.
%
When the cursor is over the constructor declaration, the fact that the
developer added a new property immediately prior is a strong hint that the
suggestion to add the parameter and initialize the property is relevant.
%
Designing tools and quick actions based on temporal context requires insights
into the common temporal edit patterns in the sequence of edits performed by
developers.
%
However, these insights are not easy to obtain through mining version control
data: the relevant fine-grained sequence of edits are lost when the developer pushes
the change as a single commit to the version control history.


\ignore{
However, to our knowledge, no IDE provides an automated tool or snippet to
perform all three of these edits at once.
\gustavo{what do you mean by all three at once? I don't think this is what we
want right? the user would perform the first edit manually, and we can
predict the next 2? Btw, VS already supports this scenario but it is using
spatial information. If the user leaves the line where he added the property,
the suggestion goes away. I think we should use this example to show exactly
the benefit of adding the temporal aspect. Even if the user goes to the next
location (parameter list), we can offer the suggestion based on the temporal
aspect. We can also say that there are many ways to apply this pattern. For
instance, some users will start from the statement? }
%

\begin{itemize}
  \item Spatial context vs temporal context 
    -- spatial context doesn't show in add param location
    -- don't show for random properties (only for the one just added)
  \item Late awareness
  \item For temporal context, tool developer needs to understand the kind of
  sequences.
\end{itemize}

Adding a snippet or tool to perform all the actions in an edit sequence
pattern is not difficult in itself.
\gustavo{I don't think we should go there... I think we should talk about detecting a pattern instead of performing it.}
%
However, there are $2$ major issues facing an toolsmith in adding such tools:
\gustavo{I think it may be risky to follow this directions... I think we should focus on the temporal aspect only. There are other techniques to mine patterns in the repository that can be used to priorize feature requests.}
%
\begin{itemize}
  \item \emph{Which edit sequence patterns should be automated?}
    Currently, there is no systematic way of discovering new edit sequence
    patterns.
    %
    Either, an toolsmith has to check feature requests or has to manually
    analyze video recordings of development sessions~\cite{Ge:ICSE:RefactoringSteps}.
    %
  \item \emph{If automated, how often is will the tool be used?}
    Once an edit sequence pattern is found, the toolsmith has to make a
    decision as to whether it is worth spending time and resources on
    automating this pattern.
    %
    Again, there is no existing technique that will automatically determine
    how often such edit sequence patterns occur in real development sessions.
    %
  \item \emph{How should these sequences be automated?}
\end{itemize}
}

To this end, we develop \technique, a technique that can aid toolsmiths in
discovering temporal edit patterns of the form 
$
      \mathsf{AddProp}(\mathsf{type}, \mathsf{propName})
\cdot \mathsf{AddConstrParam}(\mathsf{type}, \mathsf{paramName})
\cdot \mathsf{AddAssignment}(\mathsf{paramName}, \mathsf{propName})$
%, and
%how often they are performed by developers.
, and use this temporal context to improve the tool support for code editing.
%
Further, not every temporal edit pattern is a simple sequence of individual
edits.
%
For example, removing a parameter from a method declaration and then updating
all its call-sites by removing the corresponding argument is the sequence
$ 
      \mathsf{DelParam}(\mathsf{method}, \mathsf{paramName})
\cdot \mathsf{DelArg}(\mathsf{method}, \mathsf{paramName})^*
$, where the $(^*)$ stands for Kleene star.
%
In general, our temporal edit patterns are given by regular expressions over
individual edit patterns.
%
We discuss three challenges in mining temporal edit patterns.

\noindent\textbf{Level of Granularity.}
In Figure~\ref{fig:dev-session}, the edit $\version_0 \to \version_3$ plays
the role of \emph{add property} in the ``add property, add parameter, and
initialize property'' sequence.
%
However, in the development session, this edit is not a single change, but a
sequence of changes $\version_0 \to \version_1$, $\version_1 \to \version_2$,
and $\version_0 \to \version_3$.
%
To produce the above temporal edit pattern, \technique has to consider the
development session at the granularity of $\version_0 \to \version_3$ instead
of the $3$ individual fine-grained edits.

% \mohammad{what is the reason for this? is it because the edit pattern is more general if the details of the three steps are allowed to be different? If so may be good to explain rather than just state the need.}

However, $\version_0 \to \version_3$ might have to be
considered at a finer granularity in a different context.
%
If the toolsmith was exploring how developers add new properties
(not what developers do before and after adding properties), each of
$\version_0 \to \version_1$, $\version_1 \to \version_2$ and
$\version_2 \to \version_3$ is relevant.
%
\ignore{
By examining the add property edit in more fine grained manner, we were able to
discover different patterns of performing the add property action: some
developers simply type the declaration left to right and others copy-paste an
existing property and change the type and the name.
\gustavo{Should we link this paragraph to the discussion in section 5.1. We talk about this example.}
\ignore{
For example, one common recurring edit pattern is to make all properties of a
single class settable (this pattern occurs, for example, when making a class
JSON deserializable).
%
In this setting, we need to consider $\version_2 \to \version_3$ its own
separate edit and not a part of a larger edit.
}
}
Hence, depending on the scenario the toolsmith is examining, the edits
may need to be ``grouped'' or ``sub-divided'', i.e., the session needs to 
considered at different levels of granularity.
% and considering patterns among the logical edits does not work.
%
% To answer queries about different scenarios and workflows, we need to examine
% the sessions at multiple granularities.

\noindent\textbf{Level of Generalization.}
The scenario of interest not only changes the appropriate granularity of edits, but also the level of generality of a single edit. 
%
\yasharth{AST(Abstract Syntax Tree) Not introduced}
In the session, the edit $\version_0 \to \version_3$ could be
considered under different levels of generalization, e.g., ``insert an  AST node'' \priyanshu{suggestion: make it "insert any AST node" to connect with the example?},
``insert a property'', ``insert a get-set property'', etc.
%
When the toolsmith is examining the add and initialize property scenario,
it does matter that $\version_0 \to \version_3$ is the insertion of a property,
not just any AST node.
%
However,  that $\version_0 \to \version_3$ adds a get-set
property is irrelevant, only that it adds a property.
%
Therefore, apart from different levels of granularity, we also need to
consider each single edit at different levels of generalization.
\yh{I believe we did not distinguish ``insert a property'', ``insert a get-set property'' in the sketches of edit sequence pattern.}

\noindent\textbf{Temporal Summarization.}
%
\ignore{
\mohammad{the terms "temporal" and "sequential" are being used interchangeably and may be better to consistently use one to avoid confusion. It seems it is less about "temporal" but more about sequence and order-sensitivity of edits.
@Mohammad: We have had quite a bit of trouble with this nomenclature of
sequential and temporal. If you have a suggestion, we can discuss it.
}
}
%
Different developers perform the same logical edit using completely
different steps.
%
In Figure~\ref{fig:add-property-pattern}, the developer performs the edits
in the sequence add property, add constructor parameter, and add assignment.
%
However, some developers use the order add constructor parameter,
add assignment, and then, add property.
%
A toolsmith is often interested not in any single sequence, but a summary
of all sequences used by developers to perform the logical edit.
%
Hence, apart from finding the edit sequence pattern at the right granularity
and generalization in one session, we need to do so across multiple sessions
and summarize all these sequence patterns into a single temporal edit pattern 
that represents all ways of performing the same logical edit.
\priyanshu{We still create temporal edit patterns at different granularity right? I am afraid having this description may warrant a discussion later in the paper about how the templates we have generated are at the "right" granularity and generalization which is currently missing.}
%
%%% OLD STUFF %%%
\ignore{
\gustavo{I think it's better change the example here by the one
where the developer perform the same set of actions using a
different order. It will make it easier to understand.}
 \arsays{Don't know what to call this.}
\gustavo{How about using the same example. We can say that a change would be
to perform 2 add properties, then 2 parameters, then 2 assignments. The
pattern would be: AddProp*AddParameter*AddAssignment*?}
}
%
\ignore{
In many scenarios, individual temporal edit patterns may be combined into a
single, more general, temporal edit pattern.
%
For example, for add and initialize property task, different developers order
the individual edits in different ways.
%
In fact, we found instances of developers completing this task in all $6$
permutations of the three sub-steps.
%
We combine all these $6$ permutations into one temporal edit pattern
$
\{\!|  
\mathsf{AddProp}(\mathsf{type}, \mathsf{propName}),
\mathsf{AddConstrParam}(\mathsf{type}, \mathsf{paramName}),\\
\mathsf{AddAssign}(\mathsf{paramName}, \mathsf{propName})
|\!\}
$, where
$\UnorderedSeq{\cdot}$ represents an unordered collection of individual
edit patterns.
%

%
This task of summarizing individual edit sequences into a regular
expression-like temporal edit pattern is not straight-forward often needs
human guidance.
\gustavo{I think we need to improve this part, right? 
\arjun{Yes, I will change this looking at sec 5 and 6}
}
}

\ignore{
\mohammad{until now we do a good job of motivating the problem and challenges, but the intro gives no insight into the techniques used to address the challenges (just that we have created a system that does so, which may give the impression that we may be lacking in interestingness of approach).
\arjun{This is a style thing. SE papers often use this -- I haven't used it before either.}
}
}

==> old_sec2.tex <==
% ---------------
% OLD STUFF
% ---------------

\section{Motivating Example}




% We show the intricacies associated with mining edit sequence patterns using real-world concrete edit sequences.
\Cref{fig:PropertyDomain} shows two series of snapshots (\textit{versions)} of two documents, as the two respective developers are updating them in the IDE. 
It can be observed that the two developers have performed a somewhat similar sequence of code changes (\textit{edit sequence}) to update the respective documents.
In the \Cref{fig:PropertyDomain} A, at version 0 ($v_0$), the developer starts to type (character by character) the property \code{string Id} and completes the task at $v_{10}$.
Then the developer starts to type a new parameter \code{string id} to the constructor, and completes the task at $v_{16}$. 
Finally the developer completes the task of adding the assignment at $v_{20}$.
Similarly in \Cref{fig:PropertyDomain} B, the developer completes adding the new property \code{int X} at $v_{40}$, then the constructor parameter \code{int x} at $v_{42}$, and finally an assignment (at $v_{46}$). 
We can observe that the two developers performed a common sequences code changes(\textit{edits}) - add a new property to a class, then add a parameter to a constructor, and finally add an assignment inside the constructor. 


\ignore{
\begin{figure}[htbp]
  \includegraphics[scale=0.8]{figures/Fig1.pdf}
  \caption{Insert Property-Parameter-Assignment Pattern\gustavo{should we use subfigures?}}
  \label{fig:PropertyDomain}
\end{figure}
}
% \begin{figure*}[htbp]
% \centering
% \begin{minipage}{.65\textwidth}
%   \centering
%   \includegraphics[scale=0.8]{figures/Fig1.pdf}
%   \captionof{figure}{Property-Parameter-Assignment Edit Sequence Pattern}
%   \label{fig:PropertyDomain}
% \end{minipage}%
% \begin{minipage}{.35\textwidth}
%   \centering
%   \includegraphics[]{figures/Granularity.pdf}
%   \captionof{figure}{Varying granularity of edit sequences}
%   \label{fig:Granularity}
% \end{minipage}
% \end{figure*}
% \gustavo{will people understand? Version was not defined yet}
% \gustavo{before explaining the details. Give a big picture of what the example in Figure 3 shows. Then you can go and describe figures 3A and 3B}


% \gustavo{Invert? Put this in the beginning? And then explain how both sequences share the same sequence structure.}
We want to automatically infer high-level common patterns from the concrete sequence of edits developers perform in an IDE.
\gustavo{I could be interesting to have a sequence pattern representation here to make it clearer}
However, there are three major challenges: 
(a) at what granularity should we define an individual edit -- should each small change be considered a separate edit, 
or should small changes be combined to define one (bigger) edit?
%at what granularity to define an individual edit when analyzing edit sequences.
(b) how much to generalize an individual edit when trying to find identify patterns, and 
(c) how to handle the case when a general pattern can be instantiated by
variable-length edit sequences?
%at what granularity to define an individual edit when analyzing edit sequences.

\begin{enumerate}[wide, label=\bfseries Challenge-\arabic*, leftmargin=*, labelwidth=!, labelindent=0pt]
\item \textit{\textbf{Granularity of an edit: }} 
\label{challenge:granularity}
    Consider the edit
    $v_{0}\rightarrow v_{10}$ from \Cref{fig:PropertyDomain}.
    This edit can be broken down into {\em{three}} fine-grained edits
    $v_{0} \rightarrow v_{6} \rightarrow v_8\rightarrow v_{10}$ as shown
    in \Cref{fig:varying-granularity}.
    Should we work with the one coarse edit or the three fine-grained edits?
% 
%shows a coarse view of how to two documents were updated, where the versions $v_{0}$ to $v_{20}$ are summarized by 3 edits. ($v_{0}$$\rightarrow$$v_{10}$$\rightarrow$$v_{16}$$\rightarrow$$v_{20}$), and $v_{32}$ to $v_{48}$ are summarized by $v_{32}$$\rightarrow$$v_{40}$$\rightarrow$$v_{42}$$\rightarrow$$v_{48}$.
\begin{figure}[htbp]
  \includegraphics[scale=0.9]{figures/Granularity.pdf}
  \caption{Varying granularity of edit sequences}\label{fig:varying-granularity}
\end{figure}
When defining the edit pattern, recall that the coarse edit 
$v_{0}\rightarrow v_{10}$ was {\em{matched}} with
the edit $v_{32}\rightarrow v_{40}$ (\Cref{fig:PropertyDomain}).
However, at the finer-granularity, 
the edit $v_{32}\rightarrow v_{40}$ is replaced by {\em{two}} edits
$v_{32}\rightarrow v_{36}\rightarrow v_{40}$ (see \Cref{fig:varying-granularity}).
At the finer-granularity, the three edits do not ``match'' the two edits, and thus
we will miss discovering the pattern from \Cref{fig:PropertyDomain}.

%While \Cref{fig:varying-granularity} shows that the sequence of finer edits (yellow arrows) applied between $v_{0}$$\rightarrow$$v_{10}$(A), and $v_{32}$$\rightarrow$$v_{48}$(B).
%To insert the entire property in \Cref{fig:varying-granularity} A - a new property was inserted, then the \textit{get} keyword and then the \textit{set} keyword.
%On comparing the finer edit sequences (yellow arrows) in \Cref{fig:varying-granularity}, we observe that sequence A has an extra step - insert \textit{set} keyword.
%This implies that if the finer granularity is considered, no pattern will emerge from the concrete edit sequences applied between $v_{0}$$\rightarrow$$v_{20}$ and $v_{32}$$\rightarrow$$v_{48}$.

%While the finer edit sequence in \Cref{fig:varying-granularity} may not be helpful when generalizing the sequence in \Cref{fig:PropertyDomain}; 
However, the finer-granularity edits can be useful in other contexts. For example, they can help IDE designers create a feature\footnote{\url{https://github.com/dotnet/roslyn/issues/9863}} that suggests the most common \code{get}-\code{set} patterns like \smcode{\{get;\}}, \smcode{\{get;set;\}}, \smcode{\{get;private set;\}} or \smcode{\{get;internal set;\}}.
\gustavo{I am not sure if the first think to discuss is discarding... I think the problem is really how we can define these granularities... For instance, why not go one level higher? }
% Just discarding finer grained edits could results in loss of temporal information.
% The technique we describe \Cref{sec:technique} accounts for all possible granularity to define an individual edit, when surfacing the edit sequence patterns.

\item \textbf{\textit{Generalizing an edit:}}
% \gustavo{We may want to be more consistent. What's the difference between classify and generalize, pattern/category?}
\label{challenge:generalization}
To identify edit patterns from concrete edit sequences, we have to generalize individual edits so that
we can group them together.
For instance in \Cref{fig:PropertyDomain}, we grouped $v_{0}$ $\rightarrow$ $v_{10}$ (A) and $v_{32}$ $\rightarrow$ $v_{40}$ (B) by generalizing them to the same abstract edit. Similarly, we grouped $v_{10}$ $\rightarrow$ $v_{16}$ (A) and  $v_{40}$ $\rightarrow$ $v_{42}$ (B) , and we grouped $v_{16}$ $\rightarrow$ $v_{20}$ (A) and  $v_{42}$ $\rightarrow$ $v_{48}$ (B).
The individual edits that are being grouped together are not identical in all details.
For example,
the edit ($v_{0}$ $\rightarrow$ $v_{10}$) adds a \code{public} property \code{string Id}, whereas
the corresponding edit $v_{32}$ $\rightarrow$ $v_{40}$ adds a \code{private} property \code{int X}.
However, we can view both the edits as instances of ``\textit{Insert a property}'' abstract edit.
If we had instead considered the generalization ``\textit{Insert a \textbf{public} property of type \smcode{string}}'' or the generalization ``\textit{Insert a \textbf{private} property of type \smcode{int}})'', then the two edits would not be grouped together, and we would not discover the general pattern 
from the two concrete sequences in \Cref{fig:PropertyDomain}.
        On the other hand, if we generalized edits too much, say to ``\textit{Insert Code}'', then we will discover meaningless edit sequence patterns.
% The technique we describe in \Cref{sec:technique} accounts for all the possible generalizations of the edits when surfacing the common patterns.

\item \textbf{\textit{Handling repetitive edits:}} Developers often perform sequences of edits which are repetitive in nature \cite{Miltner:BluePencil}, and this can cause the same high-level pattern to be instantiated by variable-length edit sequences. 
For example, in one instance a developer renaming a variable might update the name of the variable declaration and then apply 3 repetitive edits to update all its references. 
In another instance, the renamed variable may have only 2 references, and the developer would update only 2 references. 
While these two edit sequences have different lengths, they still have the common underlying pattern - \textit{Update the Variable name} and then \textit{Update identifiers}.
% The number of times this repetitive edit is applied, depends upon how widely the variable is used.  
If such variable-length edit sequences are not generalized properly, we could explode the number of patterns mined. 
\end{enumerate}

% For instance, there could be an edit sequence pattern specific to \textit{Insert Property} of type \code{int}.

% \gustavo{We may want to delete this paragraph. At the end of section 2, we could have an example of how our entire system deals with this example in a high-level way. }
% \textcolor{red}{Our technique is not restricted to mining common edit patterns in context of larger specific edits like \textit{refactoring}, this exacerbates the the challenge of identifying the correct generalization. }


% \subsection{Granularity of an edit}





% If we consider the finer edits (yellow arrows in \Cref{fig:varying-granularity}), . Since,   \Cref{fig:varying-granularity} (A), there is this extra step of adding a \textit{set} keyword. 

% \subsection{Challenge 1: Identify the correct generalization of an edit}
% \begin{figure}
%   \includegraphics[width=\linewidth]{figures/Challege1.pdf}
%   \caption{Two separate instances where a new property is inserted}\label{fig:awesome_image1}
% \end{figure}


==> old_sec3.tex <==

\Cref{fig:techniqueOverview} shows the high-level overview of \technique. 
As input, it accepts \textit{code development sessions} and \textit{specifications}. 
A \textit{Code Development Session} are all the syntactically correct versions of the documents produced when the developer is programming in the IDE.
% The \textit{specifications} determine which \textit{edit sequence patterns} are reported by \technique. 
As \textit{specifications} the user can express the different kinds of features they desire in the patterns that \technique reports, like the number of developers that applied the pattern, the total number of instances of the pattern, or an example of edit(s) that the patterns should include. 
\technique reports all the \textit{edit sequence patterns} found in the input \textit{code development sessions} that satisfy the \textit{specifications}.
% \noindent 
% \noindent\gustavo{were do we define longer edits, like v0, v5?}% \gustavo{writing tip: when writing a paragraph like this, it's good to keep the actor of the paragraph to give flow to the text. The first 3 sentences here have diferent actors. The first sentence has `our technique', the second one has `process used for summarizing code...', and the next one has `We'.}

% \noindent A \textit{Code Development Session} is a sequence of documents $s=v_0, v_1...v_n$ created by a sequences of edits, $(v_0,v_1),(v_1,v_2),\ldots,(v_{n-1},v_n)$, applied by the developer between opening and closing the IDE application.\gustavo{were do we define longer edits, like v0, v5?}

% \technique accepts \textit{code development sessions} as input. 
% \Cref{fig:summarizer} shows the overview of the process used for summarizing code development sessions. 

% Where an \textit{edit} is a pair of versions ($v_a$, $v_b$) of the same document before the edit ($v_a$) and after the edit ($v_b$).
To represent sequences at all possible granularity (\Cref{challenge:granularity}), \technique converts the code development sessions to a \textit{Edit Graph}. %\gustavo{why?}
The \textit{Edit Graph} captures all the possible concrete edits and their \textit{sequential} (and \textit{spatial}) relationships. 
It then generates a \textit{quotient-based} summary of this \textit{Edit Graph} to obtain the \textit{Edit Sequence Summary}.%\gustavo{do we define what edit sequence summary mean? Is this the same as an edit sequence pattern?}
The \textit{Edit Sequence Summary} is a graph where the nodes represent clusters of similar edits and the edges represent the sequential or spatial relationship among the edit clusters.
This summary is computed based on a \textit{(summary-specific)} notion of equivalence among graph nodes.
To obtain this equivalence, \technique hierarchically classifies all the concrete edits at multiple levels of specificity (\Cref{challenge:generalization}).
\technique then infers \textit{Edit Sequence Patterns} from this \textit{Edit Sequence Summary}, and report the ones that match the \textit{specifications}.
% Each edge in the \textit{Edit Sequence Summary} represents an \textit{Edit Sequence pattern}, and \technique applies a \textit{growth} technique to reporta. 

\subsection{Edit Graph}
\label{sec:editGraph}
To represent edit sequences at multiple granularity (\Cref{challenge:granularity}), 
\technique generates an \textit{Edit Graph} to capture all the concrete edits and their sequential/spatial relationships.
A concrete \textit{Edit} is a pair of versions ($v_a$, $v_b$) of the same document before the edit ($v_a$) and after the edit ($v_b$). 
Each \textit{code development session} is a sequence of documents $s=v_0, v_1...v_n$ that could be created by any permutation of a non-overlapping sequences of edits like  $(v_0,v_1),(v_1,v_2),\ldots,(v_{n-1},v_n)$ or $(v_0,v_3),(v_3,v_6),\ldots,(v_{n-3},v_n)$.
\technique represents all these possible permutations using a \textit{directed acyclic multi-graph} (DAM) that captures all the versions of a document and their temporal relationship, as shown in \Cref{fig:editGraph} A.
Reasoning about edits between temporally far versions will lead to coarse-grained results (similar to commit based analysis).
While considering all the possible versions in a session entails too many edits and too many edit sequences, specially in long sessions.
To reduce the size of this DAM, \technique first filters out the coarse-grained edits that are larger than a certain \textit{threshold} size of the diff (as shown in \Cref{fig:editGraph} B).

% Moreover, our corpus contains many transient versions of the code;
% for instance, in Figure 1 (A)  we collected 9 \textit{transient} \textit{versions} of the \textit{document} when the developer types - \smcode{s}, \smcode{st}... \smcode{string}, \smcode{string I}, \smcode{string Id}, leading to \smcode{public string Id \{get; set;\}}.
% Hence, to avoid spurious results we eliminate all these transient versions and \textit{coarse-grained} edits.
% \gustavo{this paragraph should not be the first paragraph of this section. It's a distraction. I think we can just move out from the technique the entire transient part.}

\begin{figure}[htbp]
  \includegraphics[scale=0.8]{figures/EditDAG.pdf}
  \caption{Constructing the Edit Graph}\label{fig:editGraph}
\end{figure}
%\gustavo{Should we change the label of the nodes to match the way you define a edit? (e1, e2))}
% \gustavo{Again, we can just move this away from this section. We can put an implementation section where we describe additional optimizations that we did. At this point, all of this explanation is a barrier to get to the meat of the paper.}
% Each edit belongs to a sequence of edits (i.e. some edit(s) is applied before/after it) and is associated to a particular "location" in the document (i.e. modifies the content of a particular sub-tree of the AST).
% We utilize this \textit{spatial information} (location of the edit) and \textit{temporal information} (before/after edits), to weed out the transient versions of a document and the coarse-grained edits. 
% Recently, researchers Miltner et al. \cite{Miltner:BluePencil} proposed an incremental technique that uses heuristics to construct a directed acyclic multi-graph (DAM) from chronologically ordered versions of a document, as a part of a larger goal to learn context-specific repetitive edits. 
% The nodes of this graph represent versions of the document and the edges represent the edit between the two versions. 
% They also describe a procedure to reduce the size of this directed acyclic multi-graph (DAM) by discarding the transient versions and the coarse-grained edits. 
% % We implemented this technique, and constructed a reduced sized DAM (e.g., \Cref{fig:editGraph} B) for each \textit{code development session} (e.g., \Cref{fig:editGraph} A) in our corpus.\gustavo{I don't understand this.}

% \gustavo{Can we construct this from scratch? We receive the documents as input, and build the graph. Adding blue-pencil to the explanation adds complexity and makes it look like blue-pencil is a requirement for the technique.}
Next, \technique construct a \textit{Line Graph} or \textit{edge-to-vertex dual} of this DAM. 
A line graph is obtained by associating a vertex with each edge of the graph G and connecting two vertices with an edge iff the corresponding edges of G have a vertex in common~\cite{Gross_Yellen_graphs}.
We add \textbf{blue} edges when constructing the dual, to capture the sequential relationship between the concrete edits. 
For instance, the blue edge $(v_{0}, v_{10})$ $\rightarrow$ $(v_{10}, v_{16})$ in \Cref{fig:editGraph} C represents the consecutive edges $v_0$ $\rightarrow${$v_{10}$} (\textit{Insert Property}) and $v_{10}$ $\rightarrow$ $v_{16}$ (\textit{Insert Parameter}).
We further add a directed \textbf{red} edge if the source node (edit) subsumes the target node(edit).
For instance,  the edit $(v_{0}, v_{10})$ (\textit{Insert Property}) subsumes the edits $(v_{0}, v_{6})$ (\textit{Insert Property with no accessors}) and $(v_{6}, v_{10})$ (\textit{Insert get \& set}). 
These red edges that capture the spatial relationsip between the edits, allow us to identify the sequences of edits that compose to a larger edit. 
\technique constructs an edit graph for each session and merges it into a larger \textit{Edit Graph} that captures all the sessions in our corpus. 
Since edits have no relationships outside of its session, merging these graphs is straightforward.  

% This summary can be queried to identify the most frequent edit sequence patterns or find a particular patterns\gustavo{I think we need to make it consistent the term summary and pattern} based on input specifications.
% \gustavo{I found this paragraph a bit dense, and hard to understand the motivation for this complex set of steps. Maybe this is because I haven't read section 2.}
% Each edge in this summary graph represents a edit sequence pattern (e.g., \textit{"Insert Property"} $\rightarrow$ \textit{"Insert Parameter"}).
% We then apply a \textit{growth} algorithm to deduce longer edit sequence patterns and report all the edit sequence patterns applied in our corpus.


% The versions of the documents in these sessions are analyzed to generate a \textit{quotient-based Edit Sequence Summary Graph}. 



% Analysing such \textit{transient versions} could lead to spurious patterns, therefore we first remove these transient versions from our corpus. 
% A version is transient, if the location of the next edit is the same as the location of the current edit.
% Recently researchers Miltner et al. proposed a simple technique to identify such transient versions, as a part of a larger goal to learn context-specific repetitive edits on the fly in an IDE. 
% We implemented this technique and identified 18,985 non-transient versions.
% \noindent In the rest of the paper, we refer to these \nonTransientVersions non-transient documents versions created in the \noOfsessions \textit{Code Development Sessions}, as our \textit{corpus}.
% \subsection{Data Pre-processing}
% \subsection{Summarizing Edit Sequences}





% This graph contained a total of \textbf{\totalEdits} edits.
% \gustavo{Overall, I think we need a much simpler explanation for this section. This is a simple step. Given the document versions, we create a graph like in Figure 6C. It should not take 3/4 of a page to describe this procedure. Maybe start saying what is the goal of the graph. Why do you even need a graph. The goal is to capture this spatial and temporal, right? Remind me again why we want to capture the spatial relationship?}

\subsection{Multi-level classification}
\label{sec:clustering}


The \textit{Edit Graph} captures the temporal and spatial relationship among the concrete edits.
To avoid over or under generalizing the concrete edits, \technique hierarchically classifies all the concrete edits at various levels of \textit{specificity} (\Cref{challenge:generalization}).
% Our goal is to compute a quotient based summary of this \textit{Edit Graph}, that requires a notion of equivalence between the nodes of the \textit{Edit Graph} (i.e. edits). 
% While a clustering technique can be used for classifying the edits, the bigger challenge is avoiding being too specific or too general (\Cref{challenge:generalization}). 
We represent edits using four basic tree operations applied on the node $r$ in the AST of a \textit{document}:
\begin{enumerate}
    \item \textit{Insert-At}: Inserts a new AST as the $k^{th}$ child of $r$ 
    \item \textit{Delete-At}: Deletes the $k^{th}$ child of $r$
    \item \textit{Update}: Replace $r$ with a new AST 
    \item \textit{Replace-At}: \textit{Update} the $k^{th}$ child of $r$
\end{enumerate}
For instance, the edit ($v_0, v_{10}$) in \Cref{fig:PropertyDomain} (A) is a \textit{Insert-at} operation that adds a new property (\smcode{public string Id \{get; set;\}}) in the class members of \code{Node}, and the edit ($v_{10}, v_{16}$) is a \textit{Insert-at} operation that adds a new parameter (\smcode{string id}) to the constructor. 

\ignore{
\begin{figure*}
  \tikzset{
    edit/.style = {draw, rectangle, minimum width=1cm, minimum height=0.05cm},
    subsumption/.style = {color=red},
    sequencing/.style = {color=blue}
  }
  \begin{tikzpicture}
    \node[edit, xshift=+0.00cm, yshift=-0.00cm] (v0 v4) {$\version_0 \to \version_4$};

    \node[edit, xshift=+0.00cm, yshift=-1.00cm] (v0 v3) {$\version_0 \to \version_3$};
    \node[edit, xshift=+2.00cm, yshift=-1.00cm] (v1 v4) {$\version_1 \to \version_4$};

    \node[edit, xshift=+0.00cm, yshift=-2.00cm] (v0 v2) {$\version_0 \to \version_2$};
    \node[edit, xshift=+2.00cm, yshift=-2.00cm] (v1 v3) {$\version_1 \to \version_3$};
    \node[edit, xshift=+4.00cm, yshift=-2.00cm] (v2 v4) {$\version_2 \to \version_4$};

    \node[edit, xshift=+0.00cm, yshift=-3.00cm] (v0 v1) {$\version_0 \to \version_1$};
    \node[edit, xshift=+2.00cm, yshift=-3.00cm] (v1 v2) {$\version_1 \to \version_2$};
    \node[edit, xshift=+4.00cm, yshift=-3.00cm] (v2 v3) {$\version_2 \to \version_3$};
    \node[edit, xshift=+6.00cm, yshift=-3.00cm] (v3 v4) {$\version_3 \to \version_4$};

    \draw[->, subsumption] (v0 v1) edge                (v0 v2);
    \draw[->, subsumption] (v0 v1) edge[bend left=60]  (v0 v3);
    \draw[->, subsumption] (v0 v1) edge[bend left=80]  (v0 v4);
  
    \draw[->, subsumption] (v0 v2) edge                (v0 v3);
    \draw[->, subsumption] (v0 v2) edge[bend left=60]  (v0 v4);
  
    \draw[->, subsumption] (v0 v3) edge                (v0 v4);
  
    \draw[->, subsumption] (v1 v2) edge                (v0 v2);
    \draw[->, subsumption] (v1 v2) edge                (v0 v3);
    \draw[->, subsumption] (v1 v2) edge                (v0 v4);
    \draw[->, subsumption] (v1 v2) edge                (v1 v3);
    \draw[->, subsumption] (v1 v2) edge[bend right=30] (v1 v4);
  
    \draw[->, subsumption] (v1 v3) edge                (v0 v3);
    \draw[->, subsumption] (v1 v3) edge                (v0 v4);
    \draw[->, subsumption] (v1 v3) edge                (v1 v4);
  
    \draw[->, subsumption] (v1 v4) edge                (v0 v4);

    \draw[->, subsumption] (v2 v3) edge[bend left=30]  (v0 v3);
    \draw[->, subsumption] (v2 v3) edge                (v0 v4);
    \draw[->, subsumption] (v2 v3) edge                (v1 v3);
    \draw[->, subsumption] (v2 v3) edge                (v1 v4);
    \draw[->, subsumption] (v2 v3) edge                (v2 v4);
  
    \draw[->, subsumption] (v2 v4) edge[bend right=60] (v0 v4);
    \draw[->, subsumption] (v2 v4) edge                (v1 v4);
  
    \draw[->, subsumption] (v3 v4) edge[bend right=60] (v0 v4);
    \draw[->, subsumption] (v3 v4) edge[bend right=40] (v1 v4);
    \draw[->, subsumption] (v3 v4) edge                (v2 v4);
  \end{tikzpicture}
  $\qquad$
  \begin{tikzpicture}
    \node[edit, xshift=+0.00cm, yshift=-0.00cm] (v0 v4) {$\version_0 \to \version_4$};

    \node[edit, xshift=+0.00cm, yshift=-1.00cm] (v0 v3) {$\version_0 \to \version_3$};
    \node[edit, xshift=+2.00cm, yshift=-1.00cm] (v1 v4) {$\version_1 \to \version_4$};

    \node[edit, xshift=+0.00cm, yshift=-2.00cm] (v0 v2) {$\version_0 \to \version_2$};
    \node[edit, xshift=+2.00cm, yshift=-2.00cm] (v1 v3) {$\version_1 \to \version_3$};
    \node[edit, xshift=+4.00cm, yshift=-2.00cm] (v2 v4) {$\version_2 \to \version_4$};

    \node[edit, xshift=+0.00cm, yshift=-3.00cm] (v0 v1) {$\version_0 \to \version_1$};
    \node[edit, xshift=+2.00cm, yshift=-3.00cm] (v1 v2) {$\version_1 \to \version_2$};
    \node[edit, xshift=+4.00cm, yshift=-3.00cm] (v2 v3) {$\version_2 \to \version_3$};
    \node[edit, xshift=+6.00cm, yshift=-3.00cm] (v3 v4) {$\version_3 \to \version_4$};

    \draw[->, sequencing] (v0 v1) -- (v1 v2);
    \draw[->, sequencing] (v0 v1) -- (v1 v3);
    \draw[->, sequencing] (v0 v1) -- (v1 v4);

    \draw[->, sequencing] (v0 v2) -- (v2 v3);
    \draw[->, sequencing] (v0 v2) -- (v2 v4);

    \draw[->, sequencing] (v0 v3) -- (v3 v4);

    \draw[->, sequencing] (v1 v2) -- (v2 v3);
    \draw[->, sequencing] (v1 v2) -- (v2 v4);

    \draw[->, sequencing] (v1 v3) -- (v3 v4);

    \draw[->, sequencing] (v2 v3) -- (v3 v4);
  \end{tikzpicture}
  \caption{The edit graph corresponding to the session from Figure~\ref{fig:dev-session}}
  \label{fig:edit-graph}
\end{figure*}
}

\subsection{Multi-level classification}
\label{sec:clustering}

% In order to cluster the edits, they have to be featurized. 
To classify all the concrete edits, we first map the edits to an \textit{euclidean} space. 
We define a function $embed_{s}$, that maps the AST space to a \textit{characteristic vector} in n-dimensional Euclidean space, to capture the structural information of the edit.
This vector captures the occurrences of the AST \textit{node kinds} in the added and removed ASTs across the edit. 
For instance, the edit $v_{10}$$\rightarrow$$v_{16}$ (\Cref{fig:PropertyDomain} A) adds a \textit{Parameter}, a \textit{Identifier} and a \textit{PredefinedType}.
However, $embed_{s}$ does not capture the context in which the edit is performed (i.e., the location where the parameter was inserted at - constructor declaration,method declaration or a lambda expression).
\textcolor{red}{Moreover, capturing the context is crucial to differentiate \textit{rename callsite} from \textit{rename parameter}, since an edit performing a \textit{rename} will have no difference between node kinds across the edit.
Hence we define function $embed_{c}$, that maps to the occurrences of the AST \textit{node kinds} of the node $r$ (where the tree operation is applied) and its \textit{ancestors}.} 
% We parameterize $embed_{c}$ similarly. 

\begin{figure}[htbp]
  \includegraphics[scale=0.65]{figures/PropertyAST.pdf}
  \caption{AST of Property Declaration}\label{fig:propertyAST}
\end{figure}

\Cref{fig:propertyAST} shows the AST of the property declaration inserted in the edit $v_0$$\rightarrow$$v_{10}$ from our motivating example.
Using the functions $embed_{s}$ and $embed_{c}$ to featurize edits, locks us at a particular level of specificity. 
As discussed in \Cref{challenge:generalization}, very specific clusters could limit the number of mined patterns.
Therefore, we parameterize \code{embed} by a level of specificity-$d$, such that \code{embed} featurizes the added/removed AST partially - until the depth $d$. 
For instance in \Cref{fig:propertyAST}, at $d=0$ $embed_{s}$ only considers the \textit{Property declaration} node, at $d=1$ it also considers all the children (i.e. \textit{public}, \textit{int}, \textit{x}) and at $d=2$ it also considers all the grandchildren (i.e. \textit{get}, \textit{set}). 
We parameterize $embed_{c}$ similarly. Assume an edit $e$ adds zero or one subtrees ($n$) and deletes zero or one subtrees ($o$), at a node $r$ in the AST, we define:\\
$embed(e, d) = embed_{s}(n, d) - embed_{s}(o, d) + embed_{c}(r, d)$  

Using \code{embed} we featurize edits at multiple specificity ($d$), and then apply an unsupervised clustering technique (like \textit{agglomerative hierarchical clustering}) at each level, to obtain multiple classifications for an edit.
It is infeasible to use any supervised clustering techniques (like K-means), since we have no apriori knowledge about the possible kinds edits in our corpus.
We desire to classify an edit at multiple specificity ($d$), such that they have a hierarchical relationship (\textit{IS-A}) between them.
For instance, the edit $v_{0}{\rightarrow}v_{10}$ in our motivating example \textbf{is a} \textit{Insert Property with get and set}, which \textbf{is a} \textit{Insert Property}, which \textbf{is a} \textit{Insert}.

To obtain a hierarchical labelling scheme for the edits, we use a \textit{divide and conquer} like approach.
We first partition all the edits four-ways, based on the tree-operation involved in the edit - \textit{Insert, Update, Delete or Replace}.
We then apply \textit{agglomerative hierarchical clustering} on each partition where edits are featurized at $d=0$, with threshold for clustering at zero. 
Since the number of features at $d=0$ are less, keeping a strict clustering criteria eliminates spurious clusters in our further analysis. 
We now partition all the edits based on the clusters produced at $d=0$, and apply AHC on each partition by featurizing the edits at $d=1$ and increasing the threshold for clustering.
We follow the similar steps for $d=3$.
As $d$ increases, the number of edits in each partition decreases and the number of features for each edit increases, therefore we weaken the threshold for clustering to allow larger clusters.
Using such a \textit{divide and conquer} approach, we generate a hierarchical classification the of edits based on the level of specificity ($d$). 

\subsection{{Edit Sequence Summary}} 
\label{sec:EditSeqSummary}
The \textit{Edit Graph} captures the sequential and spatial relationship between the concrete edits, while the \textit{divide and conquer} clustering technique classifies edits at multiple levels of specificity. 
We now want to explore the relationships between the various classifications (or clusters) of edits.
For this purpose, we construct the \textit{Edit Sequence Summary} (shown in \Cref{fig:quotient_graph}) based on the idea of \textit{quotient graphs}. 
A \textit{quotient graph} $Q$ of a graph $G$ is a graph whose vertices are blocks of a partition of the vertices of G and where block $u$ is adjacent to block $v$ if a vertex in $u$ is adjacent to a vertex in $v$, in  G. 
An \textit{Edit Sequence Summary} is a \textit{quotient graph} such that, two blocks are adjacent iff there are \textbf{at least two} edges between the blocks in G.

\begin{figure}[htbp]
  \includegraphics[scale=0.55]{figures/QuotientGraph.pdf}
  \caption{Summary of the sequences in \Cref{fig:PropertyDomain} at $d=0$}\label{fig:quotient_graph}
\end{figure}

Each node in the \textit{Edit Sequence Summary} represents a classification of edits  and edges represent the sequential (blue edges) and spatial (red edges) relationship between these classifications. 
For instance, \Cref{fig:quotient_graph} shows the summary constructed from the concrete edit sequences in \Cref{fig:PropertyDomain} at $d=0$.
We also allow \textit{self-edges}, to capture the occurrence of a sequence of repeated edits (i.e. consecutively applied edits belong to the same edit cluster).
When constructing this summary, we compute an edge-attribute - \textit{Edit Graph Instances}, that captures a set of \textit{disconnected and edge-induced} subgraphs of the \textit{Edit Graph}, that contains all the concrete edit sequences between the classifications (partitions).
For instance, \textit{Edit Graph Instances} for \textit{Insert Property}$\rightarrow$\textit{Insert Parameter} captures two disconnected subgraphs  $E_{0-10}$ $\rightarrow$ $E_{10-16}$ and $E_{32-40}$ $\rightarrow$ $E_{40-42}$, for the two concrete edit sequences in the motivating example.


\subsection{Edit Sequences Patterns}
\label{sec:IdentifyingPatterns}
An \textit{Edit Sequence Pattern} is a ordered list of edit clusters (classifications). 
For the purpose of computing the \textit{Edit Sequence Patterns}, from the \textit{Edit Sequence Summary} we discard all the edges that capture the spatial relationship between the edits (red edges).

\subsubsection{\textbf{Identifying Edit Sequence Patterns}}
\label{sec:IdentifyingEditSequences}
Each directed edge in the \textit{Edit Sequence Summary} represents a \textit{Edit Sequence Pattern} and the edge attributes contains at least two \textit{Edit Graph Instances} capturing concrete examples of the edit sequences.
To generate longer \textit{Edit Sequence Patterns} we apply the \textit{Pattern Growth} approach. 
The \textit{Pattern Growth} approach is widely used in the frequent-subgraph mining techniques~\cite{gspan,gaston_subgraph, ffsm_subgraph}; it generates patterns by expanding the existing ones. 
We generate \textit{Edit Sequence Patterns} of length $n$ by \textit{growing} each edge in the summary graph. 
We add an adjacent edge (from the summary) to an existing \textit{Edit Sequence Pattern} if atleast two \textit{Edit Graph Instances} of the \textit{pattern}, forms a series composition with the \textit{Edit Graph Instances} of the adjacent edge. 
Given two two-terminal graphs $X$ and $Y$ , with terminals $sX$ , $tX$ , $sY$ , and $tY$ , form a new graph $G = S(X,Y)$ by identifying $s=sX$,$tX =sY$,and $t=tY$, known as \textit{series composition}~\cite{eppstein_series_parallel_graphs}.
For instance, the edge or the edit sequence pattern \textit{Insert Property}$\rightarrow$\textit{Insert Parameter} in \Cref{fig:quotient_graph} can be extended to include the edge \textit{Insert Parameter}$\rightarrow$\textit{Insert Assignment}, because the both the \textit{Edit Graph Instances} form a \textit{series composition} - $E_{0-10}$ $\rightarrow$ $E_{10-16}\rightarrow{E_{16-20}}$ and $E_{32-40}\rightarrow{E_{40-42}}\rightarrow{E_{42-48}}$. 
% Since each edge in the summary graph represents a \textit{Edit Sequence Pattern}, we apply \textit{Pattern Growth} on each to generate longer \textit{edit sequence patterns}.

\subsubsection{\textbf{Querying Specific Edit Sequence Patterns}} 
\label{sec:QueryingPatterns}
Our technique can also optionally accept some specifications as input and report the \textit{Edit Sequence Patterns} that match the specification. 
As specification, our technique accepts an example of an edit or a sequence of edits. 
We featurize the input edit(s) at various levels of specificity (as mentioned in \Cref{sec:clustering}) and find the node(s) representing the input edit(s) in the \textit{Edit Sequence Summary}. 
We then apply the algorithm mentioned in \Cref{sec:IdentifyingEditSequences} to find all the \textit{edit sequence patterns} that include these matched nodes.  
No patterns are reported, if no nodes match. 

If the specification contains only one edit, it also finds the \textit{edit sequence patterns} that perform the edit in the input specification. 
For this purpose, we utilize the \textbf{red edges} that represent the spatial relationship between the edit clusters. 
We find all the neighbors of the matched node in the \textit{Edit Sequence Summary}, w.r.t. to the spatial (red) edges. 
We then report the  \textit{Edit Sequence Pattern} that only involve these neighbor nodes.  

% We then check if the targets nodes (edits) of these outgoing edges form a amongst them. 

==> threats-to-validity.tex <==
\section{Limitations}

Works better for smaller edits than larger ones ... simple vectorization 
\technique is very general. Can extend \technique to other mining techniques like  RMiner, to accurately identify larger tasks and then use \technique to find the steps involved. 

